Graphiti: Bridging Graph and Relational Database Queries

This paper presents an automated reasoning technique for checking equivalence between graph database queries written in Cypher and relational queries in SQL. To formalize a suitable notion of equivalence in this setting, we introduce the concept of database transformers, which transform database instances between graph and relational models. We then propose a novel verification methodology that checks equivalence modulo a given transformer by reducing the original problem to verifying equivalence between a pair of SQL queries. This reduction is achieved by embedding a subset of Cypher into SQL through syntax-directed translation, allowing us to leverage existing research on automated reasoning for SQL while obviating the need for reasoning simultaneously over two different data models. We have implemented our approach in a tool called Graphiti and used it to check equivalence between graph and relational queries. Our experiments demonstrate that Graphiti is useful both for verification and refutation and that it can uncover subtle bugs, including those found in Cypher tutorials and academic papers.

==> figures/fig-correct-cypher-example.tex <==
\begin{figure}[!t]
\small
\begin{tabular}{l}
\boldMatch \texttt{(s:SENTENCE)<-[r3:SP]-(p2:PA)<-[r4:CS]-[c2:CONCEPT]} \\
\boldWhere \boldExists \{ \boldMatch \texttt{(c1:CONCEPT \{CID: 1\})-[r1:CS]->(p1:PA)-[r2:SP]->(s:SENTENCE)} \} \\
\boldReturn \texttt{c2.CID}, \boldCount(*)
\end{tabular}
\vspace{-10pt}
\caption{Standard database transformer.}
\label{fig:correct-cypher-example}
\vspace{-10pt}
\end{figure}


==> figures/fig-example-sdt.tex <==
\begin{figure}[!t]
\changed{
\[
\begin{array}{rcl}
\texttt{CONCEPT}(\mathsf{cid}, \mathsf{name}) & \to & \texttt{Concept'}(\mathsf{cid}, \mathsf{name}) \\
\texttt{CS}(\mathsf{cid, csid, src, tgt}) & \to & \texttt{Cs'}(\mathsf{cid, csid, src, tgt}) \\
\texttt{PA}(\mathsf{pid, csid}) & \to & \texttt{Pa'}(\mathsf{pid, csid)} \\
\texttt{SP}(\mathsf{pid, sid, src, tgt}) & \to & \texttt{Sp'}(\mathsf{pid, sid, src, tgt}) \\
\texttt{SENTENCE}(\mathsf{sid, pmid}) & \to & \texttt{Sentence'}(\mathsf{sid, pmid}) \\
\end{array}
\]
}
\vspace{-10pt}
\caption{Standard database transformer.}
\label{fig:example-sdt}
\vspace{-10pt}
\end{figure}


==> figures/fig-example-transpiled-new.tex <==
\begin{figure}[!t]
\centering
\small
\begin{tabular}{l}
\boldWith T1 \boldAs ( \boldSelect c1.CID \boldAs c1_CID, \ldots, s.SID \boldAs s_SID \\
\hspace{5em} \boldFrom \underline{Concept \boldAs c1 \boldJoin CS \boldAs r1 \boldJoin PA \boldAs p1 \boldJoin SP \boldAs r2 \boldJoin Sentence \boldAs s } \\ 
\hspace{5em} \boldOn c1.CID = 1 \boldAnd c1.CID = r1.SRC \boldAnd \ldots~ \boldAnd r2.TGT = s.SID ), \\
\hspace{2em} T2 \boldAs ( \boldSelect s_SID \boldFrom T1 ), \\
\hspace{2em} T3 \boldAs ( \boldSelect s.SID \boldAs s_SID, \ldots, c2.CID \boldAs c2_CID \\
\hspace{5em} \boldFrom Sentence \boldAs s \boldJoin SP \boldAs r3 \boldJoin PA \boldAs p2 \boldJoin CS \boldAs r4 \boldJoin Concept \boldAs c2 \\ 
\hspace{5em} \boldOn s.SID = r3.TGT \boldAnd \ldots~ \boldAnd r4.SRC = c2.CID ), \\
\hspace{2em} T4 \boldAs ( \boldSelect * \boldFrom T2 \boldJoin T3 \boldOn T2.s_SID = T3.s_SID ) \\
\boldSelect T4.c2_CID, \boldCount(*) \boldFrom T4 \boldGroupBy T4.c2_CID \\
\end{tabular}
\vspace{-10pt}
\caption{Transpilation result for the Cypher query.}
\label{fig:example-transpiled}
\end{figure}



==> figures/fig-methodology-diagram.tex <==
\begin{figure}
    \centering
    % https://q.uiver.app/#q=WzAsNixbMCwwLCJHIFxcdHJpYW5nbGVyaWdodCBcXFBzaV9HIl0sWzAsMSwiUl9HIFxcdHJpYW5nbGVyaWdodCBcXFBzaV97R30nIl0sWzAsMiwiUlxcdHJpYW5nbGVyaWdodCBcXFBzaV9SIl0sWzIsMCwiVF9HIl0sWzIsMiwiVF9SIl0sWzIsMSwiVF9SIl0sWzAsMSwiXFxQaGlfXFxtYXRoc2Z7c3RkfSJdLFsxLDIsIlxcUGhpX3tcXG1hdGhzZntzdGR9fV57LTF9XFxjaXJjIFxcUGhpIl0sWzAsMiwiXFxQc2kiLDIseyJjdXJ2ZSI6NX1dLFswLDMsIlFfRyJdLFsyLDQsIlFfUiJdLFszLDUsIlxcUGhpX3tcXG1hdGhzZntzdGR9fV57b30iXSxbNSw0LCJcXFBoaV97XFxtYXRoc2Z7c3RkfX1ee28sLTF9XFxjaXJjIFxcUGhpXm8iLDFdLFszLDQsIlxcUGhpXm8iLDEseyJjdXJ2ZSI6LTV9XV0=
\[\begin{tikzcd}
	{G \triangleright \Psi_G} && {T_G} \\
	{R_G \triangleright \Psi_{G}'} && {T_R} \\
	{R\triangleright \Psi_R} && {T_R}
	\arrow["{\Phi_\mathsf{std}}", from=1-1, to=2-1]
	\arrow["{\Phi_{\mathsf{std}}^{-1}\circ \Phi}", from=2-1, to=3-1]
	\arrow["\Psi"', curve={height=30pt}, from=1-1, to=3-1]
	\arrow["{Q_G}", from=1-1, to=1-3]
	\arrow["{Q_R}", from=3-1, to=3-3]
	\arrow["{\Phi_{\mathsf{std}}^{o}}", from=1-3, to=2-3]
	\arrow["{\Phi_{\mathsf{std}}^{o,-1}\circ \Phi^o}"{description}, from=2-3, to=3-3]
	\arrow["{\Phi^o}"{description}, curve={height=-30pt}, from=1-3, to=3-3]
\end{tikzcd}\]
    \caption{Diagram illustrating our verification methodology.}
    \label{fig:methodology diagram}
\end{figure}

==> figures/tab-statistics-cypher.tex <==
\begin{table}[!t]
\scriptsize
\centering
\caption{Size of Cypher queries.}
\vspace{-10pt}
\resizebox{0.75\columnwidth}{!}{
\begin{tabular}{c|cccc|cccc}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{4}{c|}{Manually-Written Cypher Size} & \multicolumn{4}{c}{GPT-Generated Cypher Size} \\ \cline{2-9} 
& Min   & Max   & Avg   & Med  & Min    & Max    & Avg   & Med   \\
\midrule
\stackoverflow & 20      & 149      & 55.4      & 43.5     & 20       & 161       & 53.3      & 40     \\
\tutorial & 12      & 77      & 31.2      & 28     & 12       & 90       & 32.0      & 28     \\
\academic & 28      & 45      & 75.0      & 66     & 47       & 109       & 82.3      & 91     \\
\verieqlset & 29      & 174      & 66.5      & 61.5     & 33       & 171       & 67.3      & 61     \\
\todo{\mediatorset} &       &       &       &      &        &        &       &      \\
\hline
\todo{Total} &       &      &       &      &       &       &      &      \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\label{tab:statistics-cypher}
\end{table}


==> figures/tab-trans-results.tex <==
\begin{table}[!t]
\footnotesize
\centering
% \caption{Experimental results. \todo{TODO: The verification time is confusing. It shows the time of verifying the maximum bound within the 1-hour time limit for equivalent benchmarks. It shows the time of finding the first counterexample for non-equivalent benchmarks. We should consider splitting the benchmarks into two groups: equivalent and non-equivalent.}}
\caption{Query transpilation results.}
\vspace{-10pt}
\begin{tabular}{c|c|cccc|cccc}
\toprule
\multirow{2}{*}{Dataset} &
\multirow{2}{*}{\# Succ} &
\multicolumn{4}{c|}{Time ($10^{-3}$s)} &
\multicolumn{4}{c}{Transpiled SQL size} \\ \cline{3-10}
                         &  & Min   & Max   & Avg   & Med  & Min   & Max   & Avg   & Med \\
\midrule
\stackoverflow & 12 & 0.7    & 5.7     & 1.7      & 1.3     & 40      & 247      & 89.1      & 64     \\
\tutorial      & 26 & 0.5    & 2.5      & 1.2       & 1.1     & 30      & 291      & 87.8      & 61.5     \\
\academic      & 7  & 1.1    & 2.7      & 1.7      & 1.5     & 82      & 201      & 133.1      & 124     \\
\verieqlset      & 60  & 0.8    & 31.4      & 2.6      & 2.0     & 48      & 347      & 128.0      & 110.5     \\
\hline
Total      & 105  & 0.5    & 31.4      & 2.1      & 1.7     & 30      & 347      & 114.0      & 99     \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\label{tab:trans-results}
\end{table}


==> sections/ack.tex <==
\section*{Acknowledgments} \label{sec:ack}

We would like to thank the anonymous reviewers of PLDI for their detailed and helpful comments on this paper. This research is supported by the \todo{Natural Sciences and Engineering Research Council of Canada (NSERC) Discovery Grant} and the \todo{National Science Foundation (NSF) Grant No. CCF-XX}.


==> sections/data-availability.tex <==
\section*{Data-Availability Statement}\label{sec:das}

The software that implements the techniques described in Section~\ref{sec:algorithm} and supports the evaluation results reported in Section~\ref{sec:eval} is available on Zenodo~\cite{artifact}.


==> stale/algo-bounded-verify-stale.tex <==
\begin{figure}[t]
    \begin{algorithm}[H]
    \begin{algorithmic}[1]
    \small
\Procedure{BoundedVerify}{$\mathcal{S}, \mathcal{GS}, \mathcal{Q}_S, \mathcal{Q}_G, N, \VC$}
  \Statex \Input{
  \begin{itemize}[itemsep=0mm]
  \item $\mathcal{S}$ - relational schema
  \item $\mathcal{GS}$ - graph schema
  \item $Q_S$ - relational SQL query
  \item $Q_G$ - Cypher graph query
  \item $\VC$ - value correspondence
  \item $N \subset \mathbb{N}$ - bound variable
  \end{itemize}}
  \Statex \Output{Either $\top$, meaning two queries $Q_G, Q_S$ are equivalent under bound $N$ or $(\bot, cex)$, meaning non-equivalent with a counter-example $cex$)}
  \State  $(\mathcal{S}', \_) \gets \mathsf{TranslateSchema}(\mathcal{GS});$ \Comment{Translate $\mathcal{GS}$ into an equivalent SQL schema $\mathcal{S'}$}
  \State $\VC' \gets \mathsf{TranslateVC}(\VC, \mathcal{GS}, \mathcal{S'});$\Comment{Translate $\VC$ into value-correspondence $\VC'$ between $\mathcal{S}$, $\mathcal{S}'$}
  \State  $Q' \gets \mathsf{TranslateQuery}(\VC', Q_{G}, \mathcal{S'});$ \Comment{Translate $Q_G$ into an equivalent SQL query $Q'$}
  \State  $\Phi \gets \mathsf{EncodeVC}(\VC', \mathcal{S}, \mathcal{S'});$ \Comment{Encode $\VC'$ as a SMT-formula}
  \State  \Return $\textsf{Check}(N, \Phi, \mathcal{S},\mathcal{S'}, Q,Q');$ \Comment{Check if $\forall D_1 :: \mathcal{S}. D_2 :: \mathcal{S'}. \Phi(D_1, D2) \implies  Q(D_1) \sim_R Q'(D_2) $}
\EndProcedure
    
\end{algorithmic}
\end{algorithm}
\caption{Pseudocode of main algorithm for bounded verification between Cypher/SQL queries.}
\label{fig:bounded-verify-stale}
\end{figure}


==> stale/algo-trans-schema-stale.tex <==
\begin{figure}
    \begin{algorithm}[H]
    \begin{algorithmic}[1]
    \small

    \Procedure{NewRelation}{$\rho, tname, attrs$}
    \Statex \Input{$\rho$: (passed by reference) mapping that resolves from node labels/edge types to relation names} 
    \Statex \Input{$tname$: name supplied for the new relation}
    \Statex \Input{$attrs$: Attribute names supplied for the new relation}
    \Statex \Output{A tuple $(name, attrs, ICs)$ with $name$ being the new relation name, $attrs$ being the attributes belonging to the new relation, and $ICs$ being the integrity constraints induced by this new relation}
    \State $name \gets \mathsf{MakeUniqueRelationName}(tname);$ \Comment{Make unique relation name based on $tname$}
    \State $\rho[tname] \gets name;$ \Comment{Update the $\rho$ mapping, passed in by reference}
    \State $attrs' \gets name.\mathtt{id} :: attrs$; \Comment{Create attributes included inside the new relation, and append the mandatory primary key attribute $name.\mathtt{id}$}
    \State $ICs \gets \mathsf{PK}(name, name.\mathtt{id}) \wedge \mathsf{Inc}(name, name.\mathtt{id}, 0);$ \Comment{Enforce auto-incr'ed PK constraint}
    \State \Return $(name, attrs', ICs);$
    \EndProcedure 
\Statex
    \Procedure{TranslateSchema}{$\mathcal{GS} = (L, T, M, A_L, A_T)$}
    \Statex \Input{$\mathcal{GS}$ - Graph database schema}
    \Statex \Output{A relational schema $\mathcal{S'}$ and a witness value-correspondence $IVC(\mathcal{GS}, \mathcal{S'})$ that justifies the equivalence between $\mathcal{GS}$ and $\mathcal{S'}$}
    \State $\rho \gets \emptyset;$
    \Comment{A mapping from node labels/edge types in $\mathcal{GS}$ to corresponding relation names in $\mathcal{S'}$}
    \State $S' \gets \emptyset;$ \Comment{New relations created in $\mathcal{S'}$}
    \State $C' \gets \top;$ \Comment{Integrity constraints on $\mathcal{S'}$ induced by the translation}
    \For{each node label $l \in L$} \Comment{Instantiate a table for every node label $l$ in $\mathcal{SG}$}
        \State $(name, attrs, ICs) \gets \mathsf{NewRelation}(\rho, l, A_L(l));$
        \State $S' \gets S' \cup \{ (name \mapsto attrs)\};$
        \State $C' \gets C' \wedge ICs$; 
    \EndFor
    \For{each edge type $t \in T$} \Comment{instantiate a table for every edge type $t$ in $\mathcal{SG}$}
    \State $name, attrs, ICs \gets \mathsf{NewRelation}(t, A_T(t));$
    \State $S' \gets S' \cup \{ (name \mapsto attrs) \}$;
    \State $(l_1, l_2) \gets M(t);$
    \State $C' \gets C' \wedge  ICs \wedge \mathsf{FK}(\rho[l_1], \rho[l_1].\texttt{id}, \rho[l_2], \rho[l_2].\texttt{id});$ \Comment{Create one foreign-key constraint per edge}
    \EndFor 
    $IVC \gets \emptyset;$ \Comment{Creation of the witness value-correspondence}
    \For{$l \in L$}
        \For{$p$ in $A_L(l)$}
            \State $IVC \gets IVC \cup \{\rho[l].p \mapsto p \}$;
        \EndFor
    \EndFor
    \For{$t \in T$}
        \For{$p$ in $A_T(t)$}
            \State $IVC \gets IVC \cup \{\rho[t].p \mapsto p \}$;
        \EndFor
    \EndFor
    \State \Return $(\mathcal{S'}:=(S', C'), IVC);$
    \EndProcedure
%Instantiate a table T for every node label T in S_G
%For every edge type T_E in S_G with a non-empty set of property keys, instantiate a table T_E in S
%Create HAS_ORDER table for the HAS_ORDER edge type.
%Introduce integrity constraints:
%Customer.id, HAS_ORDER.id, Order.id are PKs
%(Customer.id, HAS_ORDER.cust_id) is a pk-fk pair
%(Order.id, HAS_ORDER.order_id) is a pk-fk pair
%For every edge type T_E in S_G with an empty set of property keys, translate this into a (primary key, foreign key) integrity constraint in S.  (this is an optimization; we can also introduce an explicit table for 2. 
%After doing so, we get a relational schema S’ and a lookup function Lookup: {Node Label} U {Edge Type} -> Table.
    \end{algorithmic}
    \end{algorithm}
    \vspace{-10pt}
    \caption{Algorithm for naive translation of a graph schema $\mathcal{GS}$ to a relational SQL schema $\mathcal{S'}$.}
    \label{fig:schematranslate}
\end{figure}


==> stale/availability.tex <==
\section*{Data-Availability Statement}
The software that supports our proposed techniques in Section~\ref{sec:translation}, methodology in Section~\ref{sec:methodology}, and evaluation results in Section~\ref{sec:eval} will be submitted to artifact evaluation, if this paper is selected to publish at OOPSLA 2024.


==> stale/fig-dsl-schema-transformer-stale.tex <==
\begin{figure}
\centering
\small
\[
\begin{array}{l l c l}
\text{Transformer} & \transformer & ::= & O_R = O_G ~|~ \transformer \land \transformer \\
\text{Relation} & O_R & ::= & R ~|~ \proj_{\overline{a}}(O_R) ~|~ \filter_{\pred}(O_R) \\
\text{Graph} & O_G & ::= & G ~|~ \proj_{\overline{k}}(O_G) ~|~ \filter_{\pred}(O_G) ~|~ \text{Union}(\overline{O_G}) \\
\text{Predicate} & \pred & ::= & \top ~|~ \bot ~|~ a = v ~|~ k = v ~|~ \pred \land \pred ~|~ \pred \lor \pred ~|~ \neg \pred \\
\end{array}
\]
\[
\begin{array}{r c l c r c l}
G & \in & \textbf{Graphs} & & R & \in & \textbf{Relations} \\
a & \in & \textbf{Attr Names} & & k & \in & \textbf{Property Keys} \\
v & \in & \textbf{Values} \\
\end{array}
\]

\caption{DSL for expressing schema transformer (\yang{WIP. Illustrate with some examples})}
\label{fig:dsl-schema-transformer-stale}
\end{figure}


==> stale/fig-example-qa2.tex <==
\begin{figure}[H]
\centering
\begin{minipage}{\linewidth}
\centering
\begin{subfigure}{\textwidth}
\centering
\footnotesize
% customers
\begin{subfigure}[b]{0.4\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
CustomerID & CompanyName \\
\hline
0 & 'Drachenblut D...'  \\
\hline
1 & 'Ava'  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{Customers}}
\end{subfigure}
~
% orders
\begin{subfigure}[b]{0.3\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
OrderID & CustomerID \\
\hline
0 & 0  \\
\hline
1 & 0  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{Orders}}
\end{subfigure}
~
\vspace{5pt}

% orders_details
\begin{subfigure}[b]{0.4\textwidth}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
OrderID & ProductID & UnitPrice & Quantity \\
\hline
0 & 1 & 10 & 1  \\
\hline
0 & 0 & 20 & 1  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{OrderDetails}}
\end{subfigure}
~
% products
\begin{subfigure}[b]{0.3\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
ProductID & ProductName \\
\hline
0 & 'A'  \\
\hline
1 & 'B'  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{Products}}
\end{subfigure}
\vspace{-5pt}
\caption{Counterexample SQL Input databases.}
\label{fig:motivating-example-a}
\end{subfigure}
\end{minipage}


\vspace{5pt}

\hspace{-20pt}
\begin{minipage}{.4\linewidth}
\centering
\begin{subfigure}{\linewidth}
\centering
\normalsize
\begin{tikzpicture}[main/.style = {draw, circle}] 
% \node[main] (1) [below left of=1] {$C_1$}; % (CustomerID: 0, CompanyName: "Drachenblut Delikatessen")
% \node[main] (2) [below right of=1] {$C_2$}; % (CustomerID: 1, CompanyName: NULL)
% \node[main] (3) {O_1}; % (OrderID: 0)
% \node[main] (4) {O_2$}; % (OrderID: 1)
% \draw[->] (1) -- (2);

% customers

% \node[circle, draw=mycolor1] (1) at (0, 0){$C_1$}; % (CustomerID: 0, CompanyName: "Drachenblut Delikatessen")
% \node[circle, draw=mycolor1] (2) at (3, 0){$C_2$}; % (CustomerID: 1, CompanyName: NULL)
% % orders
% \node[circle, draw=mycolor2, dashed] (3) at (-1.5, 1.5){$O_1$}; % (OrderID: 0, CustomerID: 0)
% \node[circle, draw=mycolor2, dashed] (4) at (1.5, 1.5){$O_2$}; % (OrderID: 1, CustomerID: 0)
% % products
% \node[circle, draw=mycolor3, double,double distance=1pt] (5) at (3, 3){$P_1$}; % (ProductID: 0, ProdutName: '2147483648')
% \node[circle, draw=mycolor3, double,double distance=1pt] (6) at (0, 3){$P_2$}; % (ProductID: 1, ProdutName: '2147483648')

\node[circle, draw=deepred] (1) at (0, 0){DD}; % (CustomerID: 0, CompanyName: "Drachenblut Delikatessen")
\node[circle, draw=deepred] (2) at (3, 0){\scalebox{.95}{Ava}}; % (CustomerID: 1, CompanyName: NULL)
% orders
\node[circle, draw=deepblue, dashed] (3) at (-1.5, 1.5){$O_1$}; % (OrderID: 0, CustomerID: 0)
\node[circle, draw=deepblue, dashed] (4) at (1.5, 1.5){$O_2$}; % (OrderID: 1, CustomerID: 0)
% products
\node[circle, draw=deepgreen, double,double distance=1pt] (5) at (3, 3){B}; % (ProductID: 0, ProdutName: '2147483648')
\node[circle, draw=deepgreen, double,double distance=1pt] (6) at (0, 3){A}; % (ProductID: 1, ProdutName: '2147483648')


\draw[->] (1) -- (3) node [midway, above, sloped] (purchase1) {\scalebox{.5}{: PURCHASED}};
\draw[->] (1) -- (4) node [midway, above, sloped] (purchase1) {\scalebox{.5}{: PURCHASED}};
\draw[->, purple] (4) -- (5) node [midway, above, sloped] (purchase1) {\scalebox{.5}{: PRODUCT}};
\draw[->, purple] (4) -- (6) node [midway, above, sloped] (purchase1) {\scalebox{.5}{: PRODUCT}};

% \path [->] (1) edge node[above, sloped] {PURCHASED} (4);

\end{tikzpicture} 
\vspace{-5pt}
\caption{Counterexample Cypher Input graph. The DD and Ava nodes denote two customers, and A and B are two product names.}
\label{fig:motivating-example-b}
\end{subfigure}
\end{minipage}
\ \ 
\hspace{5pt}
\begin{minipage}{0.3\linewidth}
\centering
\footnotesize
\begin{subfigure}{\linewidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
ProductName & Volume \\
\hline
'A' & 20 \\
\hline
'B' & 10 \\
\hline
\ttNull & \ttNull \\
\hline
\end{tabular}
\caption{Output of SQL query.}
\end{subfigure}

\vspace{10pt}

\begin{subfigure}{\linewidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
ProductName & Volume \\
\hline
'A' & 20 \\
\hline
'B' & 10 \\
\hline
\end{tabular}
\caption{Output of Cypher query.}
\end{subfigure}
\end{minipage}

\vspace{-5pt}
\caption{The counterexample and query results.}
\label{fig:example-qa2} 
\end{figure}



==> stale/fig-example-queries.tex <==
\begin{figure}[!t]
\centering
\small

\begin{minipage}{\linewidth}
\centering

\begin{subfigure}{\linewidth}
\centering
\footnotesize
\begin{tabular}{l}
\boldSelect \texttt{c2.CID, \boldCount(*)} \boldFrom \texttt{Cs \boldAs c2, Pa \boldAs p2, Sp \boldAs s2} \\
\boldWhere \texttt{s2.PID = p2.PID \boldAnd p2.CSID = c2.CSID \boldAnd s2.SID \boldIn (} \\
\hspace{2.em} \texttt{\boldSelect s1.SID} 
\texttt{\boldFrom Cs \boldAs c1, Pa \boldAs p1, Sp \boldAs s1} \\
\hspace{2.em} \texttt{\boldWhere s1.PID = p1.PID \boldAnd p1.CSID = c1.CSID \boldAnd c1.CID = 1}
\texttt{)} \\
\boldGroupBy \texttt{CID} \\
\end{tabular}
\vspace{-5pt}
\caption{SQL query}
\label{fig:example-sql-query}
\end{subfigure}

\vspace{5pt}

\begin{subfigure}{\linewidth}
\centering
\begin{tabular}{l}
\boldMatch \texttt{($c_1$:CONCEPT \{CID:1\})-[$r_1$:CS]->($p_1$:PA)-[$r_2$:SP]->($s$:SENTENCE)} 
\boldWith \texttt{$s$} \\
\boldMatch \texttt{($s$:SENTENCE)<-[$r_3$:SP]-($p_2$:PA)<-[$r_4$:CS]-($c_2$:CONCEPT)} \\
\boldReturn \texttt{$c_2$.CID, \boldCount(*)} \\
\end{tabular}
\vspace{-5pt}
\caption{Cypher query}
\label{fig:example-cypher-query}
\end{subfigure}

\end{minipage}


\vspace{-10pt}
\caption{A non-equivalent pair of SQL and Cypher queries.}
\label{fig:example-queries}
\vspace{-10pt}
\end{figure}




==> stale/fig-example-results.tex <==
\begin{figure}[!t]
\centering
\small

\begin{subfigure}{0.4\linewidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
c2.CID & Count(*) \\
\hline
1 & 2 \\
\hline
\end{tabular}
\caption{The result of SQL query.}
\label{fig:example-sql-result}
\end{subfigure}
~
\begin{subfigure}{0.4\linewidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
c2.CID & Count(*) \\
\hline
1 & 4 \\
\hline
\end{tabular}
\caption{The result of Cypher query.}
\label{fig:example-cypher-result}
\end{subfigure}

\vspace{-5pt}
\caption{The execution results of SQL and Cypher queries.}
\label{fig:example-results} 
\vspace{-10pt}
\end{figure}




==> stale/fig-motivating-example-neo4j-correct-cypher.tex <==
\begin{figure}
\centering
\footnotesize
\begin{tabular}{l}
\boldMatch \texttt{(c:Customer \{companyName: "Drachenblut Delikatessen"\})} \\
\boldOptMatch \texttt{(o:Order)<-[:PURCHASED]-(c)} \\
% OPTIONAL MATCH (O)-[PU:E$PRODUCT]->(P:N$PRODUCT)
\boldOptMatch \texttt{(p:Product)<-[pu:PRODUCT]-(o)} \\
% \boldOptMatch \texttt{(p:Product)} \\
\boldReturn \texttt{p.productName, \boldSum(pu.unitPrice * pu.quantity)} \boldAs \texttt{volume} \\
\boldOrderBy volume \ttDesc
\end{tabular}
\vspace{-5pt}
\caption{The equivalent Cypher query of the SQL query $Q_1$ in the Figure~\ref{fig:neo4j-example}.}
\label{fig:motivating-equivalent-cypher}
\end{figure}

==> stale/fig-motivating-example-neo4j-counterexample.tex <==
\begin{figure}[H]
\centering
\begin{minipage}{\linewidth}
\centering
\begin{subfigure}{\textwidth}
\centering
\footnotesize
% customers
\begin{subfigure}[b]{0.4\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
CustomerID & CompanyName \\
\hline
0 & 'Drachenblut D...'  \\
\hline
1 & 'Ava'  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{customers}}
\end{subfigure}
~
% orders
\begin{subfigure}[b]{0.3\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
OrderID & CustomerID \\
\hline
0 & 0  \\
\hline
1 & 0  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{orders}}
\end{subfigure}
~
\vspace{5pt}

% orders_details
\begin{subfigure}[b]{0.4\textwidth}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
OrderID & ProductID & UnitPrice & Quantity \\
\hline
0 & 1 & 10 & 1  \\
\hline
0 & 0 & 20 & 1  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{orders_details}}
\end{subfigure}
~
% products
\begin{subfigure}[b]{0.3\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
ProductID & ProductName \\
\hline
0 & 'A'  \\
\hline
1 & 'B'  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{products}}
\end{subfigure}
\vspace{-5pt}
\caption{Counterexample SQL Input databases.}
\label{fig:motivating-example-a}
\end{subfigure}
\end{minipage}


\vspace{5pt}

\hspace{-20pt}
\begin{minipage}{.4\linewidth}
\centering
\begin{subfigure}{\linewidth}
\centering
\normalsize
\begin{tikzpicture}[main/.style = {draw, circle}] 
% \node[main] (1) [below left of=1] {$C_1$}; % (CustomerID: 0, CompanyName: "Drachenblut Delikatessen")
% \node[main] (2) [below right of=1] {$C_2$}; % (CustomerID: 1, CompanyName: NULL)
% \node[main] (3) {O_1}; % (OrderID: 0)
% \node[main] (4) {O_2$}; % (OrderID: 1)
% \draw[->] (1) -- (2);

% customers

% \node[circle, draw=mycolor1] (1) at (0, 0){$C_1$}; % (CustomerID: 0, CompanyName: "Drachenblut Delikatessen")
% \node[circle, draw=mycolor1] (2) at (3, 0){$C_2$}; % (CustomerID: 1, CompanyName: NULL)
% % orders
% \node[circle, draw=mycolor2, dashed] (3) at (-1.5, 1.5){$O_1$}; % (OrderID: 0, CustomerID: 0)
% \node[circle, draw=mycolor2, dashed] (4) at (1.5, 1.5){$O_2$}; % (OrderID: 1, CustomerID: 0)
% % products
% \node[circle, draw=mycolor3, double,double distance=1pt] (5) at (3, 3){$P_1$}; % (ProductID: 0, ProdutName: '2147483648')
% \node[circle, draw=mycolor3, double,double distance=1pt] (6) at (0, 3){$P_2$}; % (ProductID: 1, ProdutName: '2147483648')

\node[circle, draw=deepred] (1) at (0, 0){DD}; % (CustomerID: 0, CompanyName: "Drachenblut Delikatessen")
\node[circle, draw=deepred] (2) at (3, 0){\scalebox{.95}{Ava}}; % (CustomerID: 1, CompanyName: NULL)
% orders
\node[circle, draw=deepblue, dashed] (3) at (-1.5, 1.5){$O_1$}; % (OrderID: 0, CustomerID: 0)
\node[circle, draw=deepblue, dashed] (4) at (1.5, 1.5){$O_2$}; % (OrderID: 1, CustomerID: 0)
% products
\node[circle, draw=deepgreen, double,double distance=1pt] (5) at (3, 3){B}; % (ProductID: 0, ProdutName: '2147483648')
\node[circle, draw=deepgreen, double,double distance=1pt] (6) at (0, 3){A}; % (ProductID: 1, ProdutName: '2147483648')


\draw[->] (1) -- (3) node [midway, above, sloped] (purchase1) {\scalebox{.5}{: PURCHASED}};
\draw[->] (1) -- (4) node [midway, above, sloped] (purchase1) {\scalebox{.5}{: PURCHASED}};
\draw[->, purple] (4) -- (5) node [midway, above, sloped] (purchase1) {\scalebox{.5}{: PRODUCT}};
\draw[->, purple] (4) -- (6) node [midway, above, sloped] (purchase1) {\scalebox{.5}{: PRODUCT}};

% \path [->] (1) edge node[above, sloped] {PURCHASED} (4);

\end{tikzpicture} 
\vspace{-5pt}
\caption{Counterexample Cypher Input graph. The DD and Ava nodes denote two customers, and A and B are two product names.}
\label{fig:motivating-example-b}
\end{subfigure}
\end{minipage}
\ \ 
\hspace{5pt}
\begin{minipage}{0.3\linewidth}
\centering
\footnotesize
\begin{subfigure}{\linewidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
p.ProductName & Volume \\
\hline
'A' & 20 \\
\hline
'B' & 10 \\
\hline
\ttNull & \ttNull \\
\hline
\end{tabular}
\caption{$Q_1$'s expected output.}
\end{subfigure}

\vspace{10pt}

\begin{subfigure}{\linewidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
p.productName & volume \\
\hline
'A' & 20 \\
\hline
'B' & 10 \\
\hline
\end{tabular}
\caption{$Q_2$'s expected output.}
\end{subfigure}
\end{minipage}

\vspace{-5pt}
\caption{The counterexample and their execution results.}
\label{fig:neo4j-counterexample} 
\vspace{-10pt}
\end{figure}




==> stale/fig-motivating-example-vldb-correct-cypher.tex <==
\begin{figure}
\centering
\small
\begin{tabular}{l}
\boldMatch \texttt{($c_2$:Concept)-[:CS]->($p_2$:PA)-[$r_3$:SP]->($s$:Sentence)} \\
\boldWhere \texttt{(:Concept \{CID: 1\})-[:CS]->(:PA)-[:SP]->($s$)} \\
\boldReturn \texttt{$c_2$.CID, \boldCount(*)} \\
\end{tabular}
\vspace{-10pt}
\caption{An equivalent Cypher query.}
\label{fig:example-equivalent-cypher}
\vspace{-10pt}
\end{figure}


==> stale/fig-motivating-example-vldb-counterexample.tex <==
\begin{figure}[!t]
\centering
\begin{minipage}{\linewidth}
\centering
\begin{subfigure}{\textwidth}
\centering
\small
% Concept
\begin{subfigure}[b]{0.2\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
CID & Name \\
\hline
1 & 'Atropine'  \\
\hline
2 & 'Aspirin'  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{Concept}}
\end{subfigure}
~
% CS
\begin{subfigure}[b]{0.2\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
CID & CSID \\
\hline
1 & 0 \\
\hline
2 & 0 \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{CS}}
\end{subfigure}
~
% PA
\begin{subfigure}[b]{0.2\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
CSID & PID \\
\hline
0 & 0 \\
\hline
0 & 1 \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{PA}}
\end{subfigure}
~
% SP
\begin{subfigure}[b]{0.2\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
PID & SID \\
\hline
0 & 0 \\
\hline
1 & 0 \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{SP}}
\end{subfigure}
~
% Sentence
\begin{subfigure}[b]{0.2\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
SID & PMID \\
\hline
0 & 0  \\
\hline
1 & 0  \\
\hline
\end{tabular}
\vspace{-5pt}
\caption*{\texttt{Sentence}}
\end{subfigure}
~
\vspace{-5pt}
\caption{Input relational database.}
\label{fig:example-sql-input}
\end{subfigure}
\end{minipage}


\vspace{5pt}

\hspace{-20pt}
\begin{minipage}{.4\linewidth}
\centering
\begin{subfigure}{\linewidth}
\centering
\normalsize
\begin{tikzpicture}[main/.style = {draw, circle}] 

% Concept
\node[circle, draw=deepred] (1) at (0, 2){\scalebox{.6}{Atropine}};
\node[circle, draw=deepred] (2) at (0, 0){\scalebox{.7}{Aspirin}};
% PA
\node[circle, draw=deepblue, dashed] (3) at (2.5, 2){\scalebox{.95}{PA$_0$}};
\node[circle, draw=deepblue, dashed] (4) at (2.5, 0){\scalebox{.95}{PA$_1$}};
% Sentence
\node[circle, draw=deepgreen, double,double distance=1pt] (5) at (4.5, 2){\scalebox{1.}{S$_0$}};
\node[circle, draw=deepgreen, double,double distance=1pt] (6) at (4.5, 0){\scalebox{1.}{S$_1$}};

\draw[->] (1) -- (3) node [midway, above, sloped] (cs1) {:CS};
\draw[->] (1) -- (4) node [midway, above, sloped] (cs2) {\qquad :CS};
\draw[->] (2) -- (3) node [midway, above, sloped] (cs3) {\qquad :CS};
\draw[->] (2) -- (4) node [midway, above, sloped] (cs4) {:CS};

\draw[->] (3) -- (5) node [midway, above, sloped] (cs5) {:SP};
\draw[->] (4) -- (5) node [midway, above, sloped] (cs6) {:SP};

\end{tikzpicture} 
\vspace{-5pt}
\caption{Input graph database. Aspirin and Atropine denote two Concept nodes, PA$_0$ and PA$_1$ are two PA nodes, and S$_0$ and S$_1$ are two Sentence nodes.}
\label{fig:example-cypher-input}
\end{subfigure}
\end{minipage}
\ \ 
\hspace{5pt}
\begin{minipage}{0.3\linewidth}
\centering
\small
\begin{subfigure}{\linewidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
c2.CID & Count(*) \\
\hline
1 & 2 \\
\hline
2 & 2 \\
\hline
\end{tabular}
\caption{The output of SQL query.}
\label{fig:example-sql-output}
\end{subfigure}

\vspace{10pt}

\begin{subfigure}{\linewidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
$c_2$.CID & Count(*) \\
\hline
1 & 4 \\
\hline
2 & 4 \\
\hline
\end{tabular}
\caption{The output of Cypher query.}
\label{fig:example-cypher-output}
\end{subfigure}
\end{minipage}

\vspace{-5pt}
\caption{The counterexample and their execution results.}
\label{fig:example-counterexample} 
\vspace{-10pt}
\end{figure}




==> stale/fig-motivating-example-vldb-intermediate-sql.tex <==
\begin{figure}
\centering
\small
\begin{tabular}{l}
\boldWith T1 \boldAs ( \boldSelect c1.CID \boldAs c1_CID, \ldots, s.SID \boldAs s_SID \\
\hspace{5em} \boldFrom \underline{Concept \boldAs c1 \boldJoin CS \boldAs r1 \boldJoin PA \boldAs p1 \boldJoin SP \boldAs r2 \boldJoin Sentence \boldAs s } \\ 
\hspace{5em} \boldOn c1.CID = 1 \boldAnd c1.CID = r1.CID \boldAnd \ldots~ \boldAnd r2.SID = s.SID ), \\
\hspace{2em} T2 \boldAs ( \boldSelect s_SID \boldFrom T1 ), \\
\hspace{2em} T3 \boldAs ( \boldSelect s.SID \boldAs s_SID, \ldots, c2.CID \boldAs c2_CID \\
\hspace{5em} \boldFrom Sentence \boldAs s \boldJoin SP \boldAs r3 \boldJoin PA \boldAs p2 \boldJoin CS \boldAs r4 \boldJoin Concept \boldAs c2 \\ 
\hspace{5em} \boldOn s.SID = r3.SID \boldAnd \ldots~ \boldAnd r4.CID = c2.CID ), \\
\hspace{2em} T4 \boldAs ( \boldSelect * \boldFrom T2 \boldJoin T3 \boldOn T2.s_SID = T3.s_SID ) \\
\boldSelect T4.c2_CID, \boldCount(*) \boldFrom T4 \boldGroupBy T4.c2_CID \\
\end{tabular}
\vspace{-10pt}
\caption{The transpilation result for the Cypher query in Figure~\ref{fig:example-cypher-query}.}
\label{fig:example-irq}
\vspace{-10pt}
\end{figure}


==> stale/fig-sdt-rdt-diagram.tex <==
\begin{figure}
    \centering
% https://q.uiver.app/#q=WzAsNixbMCwwLCJHIFxcdHJpYW5nbGVyaWdodCBcXFBzaV9HIl0sWzAsMywiRCBcXHRyaWFuZ2xlcmlnaHQgXFxQc2lfUiJdLFsxLDEsIkQnIFxcdHJpYW5nbGVyaWdodCBcXFBzaV97Uid9Il0sWzQsMSwiVF97Uid9Il0sWzMsMCwiVF9HIl0sWzMsMywiVF9SIl0sWzAsMSwiXFxQaGkiLDEseyJjdXJ2ZSI6M31dLFswLDIsIlxcUGhpX3tcXG1hdGhzZntzc3R9fSIsMSx7ImN1cnZlIjoxfV0sWzIsMCwiXFxQaGlfe1xcbWF0aHNme3NzdH19XnstMX0iLDEseyJjdXJ2ZSI6MX1dLFsyLDEsIlxcUGhpJz1cXFBoaV97XFxtYXRoc2Z7c3N0fX1eey0xfVxcY2lyY1xcUGhpIiwxXSxbMiwzLCJRX3tSJ309XFxQaGlfe1xcbWF0aHNme3NzdH19XnstMX1cXGNpcmMgUV9HIiwxXSxbMCw0LCJRX0ciLDFdLFsxLDUsIlFfUiIsMV0sWzQsNSwie1xcY29sb3J7Ymx1ZX1cXHVuZGVyc2V0e1xcZXF1aXZ9ez99fSIsMSx7ImN1cnZlIjotMywic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCwzLCJcXGVxdWl2IiwxLHsiY3VydmUiOi0zLCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJkYXNoZWQifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDUsIntcXGNvbG9ye2JsdWV9XFx1bmRlcnNldHtcXGVxdWl2fXs/fX0iLDEseyJjdXJ2ZSI6LTQsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d
\[\begin{tikzcd}
	{G \triangleright \Psi_G} &&& {T_G} \\
	& {R' \triangleright \Psi_{R'}} &&& {T_{R'}} \\
	\\
	{R \triangleright \Psi_R} &&& {T_R}
	\arrow["\Phi"{description}, curve={height=18pt}, from=1-1, to=4-1]
	% \arrow["{\sdt}"{description}, curve={height=6pt}, from=1-1, to=2-2]
	\arrow["{\sdt}"{description}, from=1-1, to=2-2]
	% \arrow["{\Phi_{\mathsf{sdt}}^{-1}}"{description}, curve={height=6pt}, from=2-2, to=1-1]
	% \arrow["{\Phi'=\Phi ~\circ~ \Phi_{\mathsf{sdt}}^{-1}}"{description}, from=2-2, to=4-1]
	\arrow["{\rdt}"{description}, from=2-2, to=4-1]
	% \arrow["{Q_{R'}=Q_G ~\circ~ \Phi_{\mathsf{sdt}}^{-1}}"{description}, from=2-2, to=2-5]
    \arrow["{Q_{R'}}"{description}, from=2-2, to=2-5]
	\arrow["{Q_G}"{description}, from=1-1, to=1-4]
	\arrow["{Q_R}"{description}, from=4-1, to=4-4]
	\arrow["{{\color{blue}\underset{\equiv}{?}}}"{description}, curve={height=-18pt}, dashed, no head, from=1-4, to=4-4]
	\arrow["\equiv"{description}, curve={height=-18pt}, dashed, no head, from=1-4, to=2-5]
	\arrow["{{\color{blue}\underset{\equiv}{?}}}"{description}, curve={height=-24pt}, dashed, no head, from=2-5, to=4-4]
\end{tikzcd}\]
\vspace{-10pt}
\caption{\changed {A diagram illustrating our verification methodology.}}
\vspace{-10pt}
\label{fig:sdt-rdt-diagram}
\end{figure}




==> stale/fig-sst-rules-ebproof.tex <==
\begin{figure}
\small
    \centering

    \begin{prooftree}
        \Infer0[Init]{\mathcal{S_G} \vdash (\emptyset, \emptyset), (\emptyset \to \emptyset)}
    \end{prooftree}
    \\\vspace*{0.1in}
    \begin{prooftree}
        \hypo{\mathcal{S}_G = (N_T, E_T) \vdash \mathcal{S}_R, M}
        \hypo{\nodeType \in N_T}
        \hypo{k_1, ..., k_m \in \keys(\nodeType)}
        \hypo{l_n = \lbl(\nodeType)}
        \Infer4[Infer-Node]{ (N_T \setminus \{\nodeType\}, E_T) \vdash \mathcal{S}_R[l_n \mapsto [k_1,...,k_m], ICs(\nodeType)], M[\nodeType \mapsto l_n]}
    \end{prooftree}
    \\\vspace*{0.1in}
    
    \begin{prooftree}
        \hypo{\mathcal{S}_G = (N_T, E_T) \vdash \mathcal{S}_R, M}
        \hypo{\edgeType \in E_T}
        \hypo{k_1, ..., k_m \in \keys(\edgeType)}
        \hypo{l_e = \lbl(\edgeType)}
        \Infer4[Infer-Edge]{(N_T, E_T \setminus \{\edgeType\})\vdash \mathcal{S}_R[l_e \mapsto [k_1,...,k_m], ICs(\edgeType)], M[\edgeType \mapsto l_e]}
    \end{prooftree}\\
    \vspace*{0.1in}
    \text{Integrity Constraint for a node type $\nodeType$}: $ICs(\nodeType) = \text{PK}(\lbl(\nodeType), \mathtt{id})$ \\ 
    \vspace*{0.1in}
    \text{Integrity Constraint for an edge type $\edgeType$}:
    $ICs(\edgeType) = \text{PK}(\lbl(\edgeType), \mathtt{id}) \wedge \text{FK}(\lbl(\mathsf{src}(\edgeType)), \todo{\mathtt{sid}(t_e)}) \wedge \text{FK}(\lbl(\mathsf{dst}(\edgeType)), \todo{\mathtt{tid}(t_e)})$
    \vspace*{0.1in}
    \caption{Rules for constructing an SST from a graph schema $\mathcal{S}_G$ to an induced relational schema $\mathcal{S}_R$.}
    \label{fig:sst-rules}
\end{figure}

\begin{figure}
\small
    \centering
    \begin{prooftree}
        \Infer0[B-Init]{\mathcal{S}_R \vDash (\emptyset, \emptyset, \emptyset, \emptyset), (\emptyset \mapsto \emptyset) }
    \end{prooftree}\\
    \vspace*{0.1in}
    \begin{prooftree}
        \hypo{\mathcal{S}_R = (S, C) \vdash (V_T, E_T), W}
        \hypo{(A \mapsto [K_1,...,K_m]) \in S}
        \hypo{\todo{l_A = \mathsf{UniqueName}(A)}}
        \Infer3[B-Infer-Relation]{(S - (A, [K_1,...,K_m]), C) \mapsto (V_T \cup (l_A, K_1, ..., K_m)), W[A \mapsto (l_A, K_1, ..., K_m)]}
    \end{prooftree}\\
    \vspace*{0.1in}
    \begin{prooftree}
        \hypo{\mathcal{S}_R = (S, C) \vdash (V_T, E_T), W} 
        \hypo{\mathsf{FK}(A, t)}
    \end{prooftree}
    
    \textbf{\todo{Ruijie: TODO add more stuff here}}
    \caption{Rules for constructing a (reverse) SST from a relational schema $\mathcal{S}_R$ to a graph schema $\mathcal{S}_G$.}
    \label{fig:backward-sst-rules}
\end{figure}

==> stale/fig-trans-query-stale.tex <==
\begin{figure}[!t]
\centering
\small
    \begin{prooftree}
        \hypo{DB :: \mathcal{GS}}
        \hypo{\VC \vdash P \transpathpattern [R_1, T_1, \ldots, R_n]}
        \Infer2[Trans-Match]{\VC \vdash \mathsf{Match}(DB, P) \transquery R_1 \bowtie_{\phi_1} T_1 \bowtie_{\phi_2} \ldots \bowtie_{\phi_{2n-1}} R_n }
    \end{prooftree}

    \begin{prooftree}
        \hypo{DB :: \mathcal{GS}}
        \hypo{\VC \vdash P_1 \transpathpattern JS_1}
        \hypo{\VC \vdash P_2 \transpathpattern JS_2}
        \Infer2[Trans-OptMatch]{\VC \vdash \mathsf{OptMatch}(DB, P_1, P_2) \transquery JS_1, JS_2}
    \end{prooftree}

    \begin{prooftree}
        \hypo{\VC \vdash G \transquery Q}
        \hypo{\VC \vdash \phi_C \transpred \phi_S}
        \Infer2[Trans-Filter]{\VC \vdash\mathsf{Filter}(G, \phi_C) \transquery \sigma(Q, \phi_S) }
    \end{prooftree}

    \begin{prooftree}
        \hypo{\neg \mathsf{hasAgg}(\overline{E})}
        \hypo{\VC \vdash G \transquery Q}
        \hypo{\begin{array}{c}
        \VC \vdash E_i \transexpr E_i' \text{ for } 1\leq i \leq |\overline{E}| \\ 
        \VC \vdash F_i \transexpr F_i' \text{ for }1\leq i \leq |\overline{F}| 
        \end{array}}
        \Infer3[Trans-With]{\VC \vdash \mathsf{With}(G, \overline{E}, \overline{F}) \transquery \Pi_{\overline{\rho_{F_i'}(E_i')}}(Q) }
    \end{prooftree}

    \begin{prooftree}
    \hypo{
    \begin{array}{c}
        \mathsf{hasAgg}(\overline{E}) \\
        \overline{H} = \mathsf{nonAgg}(\overline{E})
    \end{array}
    }
    \hypo{\VC \vdash G \transquery Q}
    \hypo{
    \begin{array}{c}
    \VC \vdash E_i \transexpr E_i’ \text{ for }1\leq i \leq |\overline{E}| \\ 
    \VC \vdash F_i \transexpr F_i' \text{ for }1\leq i \leq |\overline{F}|
    \end{array}}
\Infer3[Trans-With-Agg]{\VC \vdash \mathsf{With}(G, \overline{E}, \overline{F}) \transquery 
\mathsf{GroupBy}(Q, \overline{H}, \overline{\rho_{F_i'}(E_i')}, \top)}
\end{prooftree}

    \begin{prooftree}
        \hypo{\neg \mathsf{hasAgg}(\overline{E})}
        \hypo{\VC \vdash G \rightarrow Q}
        \hypo{\begin{array}{c}
             \VC \vdash E_i \transexpr E_i'\text{ for }1\leq i \leq |\overline{E}|\\
             \VC \vdash F_i \transexpr F_i' \text{ for }1\leq i \leq |\overline{F}| 
        \end{array}}
        \Infer3[Trans-Return]{\VC \vdash \mathsf{Return}(G, \overline{E}, \overline{F}) \transquery \rho_{\overline{E}'}(\Pi_{\overline{F}'}(Q))}
    \end{prooftree}
    
\begin{prooftree}
    \hypo{
    \begin{array}{c}
     \mathsf{hasAgg}(\overline{A}) \\ 
     \overline{H} = \mathsf{nonAgg}(\overline{E}
     \end{array}}
    \hypo{\VC \vdash G \transquery Q}
    \hypo{\begin{array}{c}
         \VC \vdash E_i \transquery E'_i \text{ for }1\leq i \leq |\overline{E}| \\ 
         \VC \vdash F_i \transquery F'_i \text{ for }1\leq i \leq |\overline{F}| 
    \end{array}}
    \Infer3[Trans-Return-Agg]{\VC \vdash \mathsf{Return}(G, \overline{E}, \overline{F}) \transquery \mathsf{GroupBy}(Q, \overline{E}, \overline{\rho_{F_i'}(E_i')}, \top)} 
\end{prooftree}

    \begin{prooftree}
        \hypo{\VC \vdash G \transquery Q}
        \Infer1[Trans-Distinct]{\VC \vdash \mathsf{Distinct}(G) \transquery \mathsf{Distinct}(Q)}
    \end{prooftree}

    \begin{prooftree}
        \hypo{\VC \vdash G \transquery Q}
        \hypo{}
    \end{prooftree}
    \caption{Inference rules used by the $\mathsf{TranslateQuery}$ procedure to translate Cypher queries into SQL.}
    \label{fig:trans-query-stale}

%\irulelabel{a}{b}{c}

\end{figure}


==> stale/fig-trans-syntax.tex <==
\begin{comment}
\begin{figure}
\centering
\small
\changed {
\[
\begin{array}{l l c l}
\text{Transformer} & T & ::= & R \gets Q ~|~ T ~T \\
\text{Query} & Q & ::= &  \sfReturn(\sfMatch(\pattern, \pred), \overline{E}, \overline{k}) ~|~ \sfUnionAll(Q, Q) \\ 
\text{Path Pattern} & \pattern & ::= & (X, l) ~|~ (X, l), (X, l, d), \pattern \\ 
\text{Direction} & d & ::= & \leftrightarrow ~|~ \rightarrow ~|~ \leftarrow \\ 
\text{Expression} & E & ::= & k ~|~ v ~|~  E \arithop E \\ 
\text{Predicate} & \pred & ::= & \top ~|~ \bot ~|~ E \odot E ~|~ \pred \land \pred ~|~ \pred \lor \pred ~|~ \neg \pred \\ 
\text{Arithmetic Op} & \arithop & ::= & + ~|~ - ~|~ \times ~|~ / \\ 
\text{Logic Op} & \logicop & ::= & \leq ~|~ < ~|~ = ~|~ \neq ~|~ > ~|~ \geq 
\end{array}
\]
\[
\begin{array}{c}
R \in \textbf{Table Names} \quad
X \in \textbf{Node/Edge Names} \quad
l \in \textbf{Labels} \quad
k \in \textbf{Property Keys} \quad
v \in \textbf{Values} \\
\end{array}
\]
}

\vspace{-10pt}
\caption{Syntax of the database transformer.}
\label{fig:transformer-syntax}
\vspace{-10pt}
\end{figure}
\end{comment}

\begin{figure}
    \centering
    
    \begin{mdframed}
\small
\[
\hspace{-10pt}
\begin{array}{c}

\begin{comment}
    
V = v U V’      T(v) = l_1, …, K_1,..., K_n) P(v)(k_i)=v_i    (V’, Psi) —/-> L
—----------------------------[translate-node]
(V,Psi) —-/-> R_l(k_1\to v_1,...,k_n \to v_n)

E = (u, v) U E’    T(e)=l_1,K_1,...,K_n) P(e)(k_i)=v_i (E’, Psi) —--/-> L
—----------------------------[translate-edge]
(E,Psi)-----/-> R_l(k_1\to v_1,...,K_m \to v_m)

\end{comment}

\irulelabel
{
\begin{array}{cccc}
     G = (V, E, P, T) & 
     V = \{v\} \cup V' &
     \begin{array}{c}
        T(v) = (l, K_1,...,K_n) \\
        \forall i. P(v, k_i) = v_i)
     \end{array} & 
     ((V', E, P, T), \gschema) \circlearrowleft F'
\end{array}
}
{
    (G, \gschema)\circlearrowleft l(K_1:v_1,...,K_n:v_n) \cup F'
}
{
    \textsc{ToHorn-Node}
} \\ 
\\

\irulelabel
{
\begin{array}{cccc}
     G = (V, E, P, T) & 
     E = \{e\} \cup E' &
     \begin{array}{c}
        T(e) = (l, K_1,...,K_n) \\
        \forall i. P(e, k_i) = v_i)
     \end{array} & 
     ((V, E', P, T), \gschema) \circlearrowleft F'
\end{array}
}
{
    (G, \gschema) \circlearrowleft l(K_1:v_1,...,K_n:v_n) \cup F'
}
{
   \textsc{ToHorn-Edge}
}
\\ \\

\irulelabel
{
\begin{array}{cc}
     F = r(K_1:v_1,...,K_n:v_n) \cup F' &
     \gschema = (T_N, T_E) \\
     t = (r, K_1:v_1, ..., K_n:v_n) \in T_N & 
     (F', \gschema) \circlearrowright (V', E', P', T')
\end{array}
}
{
    (F, \gschema) \circlearrowright (V'\cup \{ \mathsf{Name}(K_1) \}, E', P'\cup\{(\mathsf{Name}(K_1), K_i) \mapsto v_i\} , T' \cup \{\mathsf{Name}(K_1) = t\})
}
{
\textsc{FromHorn-Node}
} \\ \\

\irulelabel
{
\begin{array}{cc}
     F = r(K_1:v_1,...K_n:v_n) \cup F' & 
     \gschema = (T_N, T_E) \\ 
     t = (r, K_1:v_1,...,K_n:v_n) \in T_E & 
     (F', \gschema) \circlearrowright (V', E', P', T') \\ 
     \mathsf{Name}(K_2), \mathsf{Name}(K_3) \in V'
\end{array}
}
{
    (F, \gschema) \circlearrowright (V', E' \cup \{ \mathsf{Name}(K_1) \}, P'\cup\{ (\mathsf{Name}(K_1), K_i) \mapsto v_i\} , T'\cup\{ \mathsf{Name}(K_1) \mapsto t \})
}
{
\textsc{FromHorn-Edge}
}
\\ \\ 
\irulelabel
{
\text{\todo{TODO}}
}
{
\text{\todo{TODO}}
}
{
\textsc{ToHorn-Relational}
}
\\ \\ 
\irulelabel
{
\text{\todo{TODO}}
}
{
\text{\todo{TODO}}
}
{
\textsc{FromHorn-Relational}
}
\end{array}
\]
\end{mdframed}

    \caption{Rules for translation between a relational database instance $R$ or a graph database instance $G$ and a set of datalog facts $F$.}
    \label{fig:instance-to-datalog}
\end{figure}

==> stale/figure-BuildGraph.tex <==
\begin{figure}
\raggedright
\emph{The $\mathsf{BuildGraph}(G, PP)$ function.} \\[0.05in]
\hrule
\vspace{0.05in}
\textbf{Input}: Property graph $G = (N, E, P, T)$ and path pattern $PP$ \\ 
\textbf{Output}: List of subgraphs $L := [G_1,...,G_n]$ such that:
\begin{enumerate}
    \item $\forall 1 \leq i \leq n.$ $G_i$ is a subgraph of $G$
    \item Each graph in $L$ is unique, i.e. $\forall 1\leq i, j \leq n . G_i \neq G_j$
\end{enumerate}
%\begin{enumerate}[leftmargin=*]
%\item Suppose that $\pattern$ is a node pattern, i.e., $\pattern = \nodepattern = (X, l)$, and $\mathsf{List}(N)$ is a list containing the same nodes from $N$.
% \[
% \small
% \begin{array}{l}
% \mathsf{BuildGraph}(\pattern, G) = \sfmap(\lambda n. (\set{n}, \emptyset, P[[n] \mapsto [X]], T[[X] \mapsto [l]]), \sfFilter(\lambda n. T[n] = l, \mathsf{List}(N))) \\
% \end{array}
% \] if $PP =NP$
% \\
% \[
% \small
% \begin{array}{l}
% \mathsf{BuildGraph}(\pattern, G) = \sffoldl(\lambda gs. \lambda g. gs \doubleplus \sfmap(\lambda pg. \sfMerge(pg, g), \mathsf{PreGraph}(\mathsf{headNode}(g))), [], \mathsf{BuildGraph}(\pattern')) \\
% \end{array}
% \] if $PP=NP\, EP\, PP'$



%\item Suppose that $\pattern$ is a relationship pattern, i.e., $\pattern = \nodepattern, \edgepattern, \pattern' = (X_1, l_1), (X_2, l_2, d_2), \pattern'$. Let $\mathsf{headNode}(g')$ denote a node corresponds to the node pattern $\sfHead(\pattern') = (X_3, l_3)$ where the graph $g'$ is obtained by matching the relationship pattern $\pattern'$.
%For any node $n_3 = \mathsf{headNode}(g')$, we can find a list of graphs $\mathsf{PreGraph}(n_3)$ where, for any graph $pg \in \mathsf{PreGraph}(n_3)$, $pg = (\set{n_1, n_3}, \set{e_2}, P[[n_1, e_2, n_3] \mapsto [X_1, X_2, X_3]], T[[X_1, X_2 X_3] \mapsto [l_1, l_2, l_3]])$ in which $n_1, e_2, n_3$ corresponding to the patterns $(X_1, l_1), (X_2, l_2, d_2), (X_3, l_3)$, respectively, and the edge $e_2$ connects the source node $n_1$ and the target node $n_3$.

\vspace{-10pt}
$$
\mathsf{BuildGraph}(\pattern, G) = \left\{
\begin{array}{ll}
\sfmap(\lambda n. (\set{n}, \emptyset, P[[n] \mapsto [X]], T[[X] \mapsto [l]]), &\\
\hspace{5em} \sfFilter(\lambda n. T[n] = l, \mathsf{List}(N))) \hspace{8.5em} \text{if}~ \pattern = \nodepattern & \\
\vspace{-10pt} &\\
\sffoldl(\lambda gs. \lambda g. gs \doubleplus \sfmap(\lambda pg. \sfMerge(pg, g), \mathsf{PreGraph}(\mathsf{headNode}(g, PP))),  & \\
\hspace{5em} [], \mathsf{BuildGraph}(\pattern')) \hspace{8em}  \text{if}~ \pattern = \nodepattern, \edgepattern, \pattern' & \\
\end{array}
\right.
$$

%$$\mathsf{PreGraph}(n) = \todo{... TODO}$$
%$$\mathsf{headNode}(G) = \todo{... TODO}$$
%\end{enumerate}

\caption{Definition of the $\mathsf{BuildGraph}(-)$ primitive used in the definition of pattern matching semantics in Cypher. If $G$ is a graph matched by the path pattern $PP$, then $\mathsf{headNode}(G, PP)$ returns the node in $G$ corresponding to the first node pattern in $PP$. If the path pattern is of form $PP = NP, EP, PP'$ and $\mathsf{head}(PP')=NP'$, then $\mathsf{PreGraph}(NP)$ returns a list $L$ of subgraphs such that each subgraph in $L$ matches the pattern $NP, EP, NP'$.}




\label{fig:fig-BuildGraph}
\end{figure}


==> stale/impl.tex <==
\section{Implementation} \label{sec:impl}

We have implemented the proposed techniques as a new tool called \tool, which can be used for both query transpilation and equivalence checking:
\begin{itemize}[leftmargin=*]
\item \textbf{Query transpilation.}
Given a Cypher query $Q_G$ over schema $\gschema$, \tool infers the standard schema transformer $\sdt$ and transpiles $Q_G$ to a SQL query that is equivalent to $Q_G$ modulo $\sdt$. 
\item \textbf{Equivalence verification.} \tool can also be used to check equivalence between a Cypher and a SQL query modulo a user-provided schema transformer. To do so,  \tool first transpiles the graph query to a SQL query over the induced relational schema and then leverages the \verieql tool~\cite{verieql-oopsla24} for checking equivalence between the two relational queries. 
\end{itemize}

\bfpara{Pre-processing and optimizations for query transpilation.}
While \tool closely follows the techniques presented in Section~\ref{sec:translation} to transpile Cypher queries to SQL, it leverages several pre-processing and optimization techniques to reduce the size of SQL queries.
Since \tool translates path patterns in Cypher to a sequence of join operations in SQL, it may generate a SQL query with many join operations from one Cypher query. To reduce the number of join operations in the translated code, \tool pre-processes the Cypher query to merge multiple short path patterns that share common nodes into a longer pattern and discard unused nodes in the pattern when translating it to join operations. 

% As an example, consider two patterns, namely $\texttt{(n1:Person)-[:ACTED\_IN]->(m:Movie)}$ and $\texttt{(n2:Person)-[:DIRECTED]->(m)}$, that share a common node \texttt{m}. We can merge them into a longer path pattern as follows:
% \[
% \texttt{(n1:Person)-[:ACTED\_IN]->(m:Movie)<-[:DIRECTED]-(n2:Person)}
% \]
% This pre-processing is useful, because it allows \tool to discard more unused nodes in the pattern when translating it to join operations in SQL. For instance, if the movie information is not queried but only ``connects'' actors to the director, the merged pattern can be translated into SQL joins $\rename_{\texttt{n1}}(\texttt{Person}) \ijoin \texttt{ACTED\_IN} \ijoin \texttt{DIRECTED} \ijoin \rename_{\texttt{n2}}(\texttt{Person})$ that do not involve the movie table.
% As another optimization, \tool also propagate constants on default property keys to remove unnecessary joins in the translated SQL queries. For example, the Cypher query
% \[
% \boldMatch \ \texttt{(n1:Person \{id: 1\})-[e:ACTED_IN]->(m:Movie)} \ \boldReturn \ \texttt{m.name}
% \]
% can be directed translated to $\filter_{\texttt{ACTED\_IN.pid} = 1}(\texttt{ACTED\_IN} \ijoin_{\pred} \rename_{\texttt{m}}(\texttt{Movie}))$ without joining the \texttt{Person} table, where $\pred$ is the join predicate that connects that \texttt{ACTED_IN} and \texttt{Movie} tables.


\bfpara{Leveraging \verieql.} As mentioned earlier, \tool leverages \verieql~\cite{verieql-oopsla24} to check equivalence between two relational queries. We choose \verieql as a back-end because it handles a broader subset of SQL compared to other tools~\cite{cosette,mediator-popl18} and can provide counterexamples as a bounded model checker. However, since the original version of \verieql does not support queries over different schemas, we have extended it to reason about queries over different schemas as follows:
Given two queries $Q_1, Q_2$, we first create  a pair of symbolic relational databases $D_1, D_2$ that satisfy the residual schema transformer. Then, we use \verieql to symbolically execute $Q_1, Q_2$ over these symbolic database instances and use an SMT solver to check whether the symbolic outputs are the same modulo renaming and re-ordering of columns. 







% \bfpara{Optimization for query transpilation.}
% We apply three heuristic optimization rules to reduce the complexity of translated SQL queries, which accelerate bounded equivalence checking. The first optimization rule shrinks path patterns by directly linking edges around some middle nodes. For instance, the pattern $\texttt{(n1:Person)-[:ACTED\_IN]->(m:Movie)<-[:DIRECTED]-(n2:Person)}$ can be translated into a shorter join chain, i.e., $\rename_{\texttt{n1}}(\texttt{Person}) \ijoin_{\pred_1} \texttt{ACTED\_IN} \ijoin_{\pred_2} \texttt{DIRECTED} \ijoin_{\pred_3} \rename_{\texttt{n2}}(\texttt{Person})$. The second optimization rule merges two patterns into a longer one where those two patterns share a common node with the same variable name, e.g., two patterns $\texttt{(n1:Person)-[:ACTED\_IN]->(m:Movie)}$ and $\texttt{(n2:Person)-[:DIRECTED]->(m)}$ could be rewritten as the aforementioned pattern. This optimization rule functions as query rewriting before applying the first optimization rule. 
% The last rule employs constants to represent nodes whose default property keys are determined by predicates. For instance, $\mathsf{Match}((n1, \mathsf{Person}), (e, \mathsf{ACTED\_IN}, \rightarrow), (m, \mathsf{Movie}), n1.\texttt{id} = 1)$ could be translated as $\filter_{\texttt{ACTED\_IN.pid = 1}}(\texttt{ACTED\_IN} \ijoin_{\pred} \rename_{\texttt{m}}(\texttt{Movie}))$.

% \bfpara{Automated reasoning for SQL queries over different schemas.}
% We use \verieql to verify equivalence between a SQL query translated from Cypher and another query originally designed in SQL. To this end, \verieql first instantiates databases with respect to a bound and two relational schemas that SQL queries conform to. Then, user-provided schema transformers can be encoded as formulas based on the database instances. With those database instances and formulas, \verieql is able to check equivalence of a Cypher query and a SQL query over different schemas.



% \todo{We have implemented our approach in a tool named \tool. \tool consists of three main components:

% \begin{itemize}
%     \item A \emph{transpiler} that translates a user-supplied (Cypher schema, Cypher query) pair to an equivalent (relational schema, SQL query)  pair using standard schema transformers and our syntax-directed translation scheme. 
%     \item An \emph{input specification format} and corresponding parser, which allows the user to specify inputs to the Cyper-SQL equivalence checking problem. In particular, it allows the user to specify the graph-relational schema transformer $\Phi$ (Figure~\ref{fig:sst-rst-diagram}) as a set of Cypher queries, and checks whether such a specification is allowed (in the sense that the induced schema of $\Phi$ must be the input relational schema $\schema_R$, but not an arbitrary relational schema).
%     \item A \emph{bounded equivalence checker} that checks the equivalence between a Cypher query and a SQL query given a user-supplied bound $N$ that bounds the number of rows in each table of the input database instances. To achieve this, we extend an existing bounded equivalence checker called \verieql \cite{verieql-oopsla24}  that checks whether two SQL queries are equal on the same input schema to work on two different input schemas. We then use the transpiler to translate Cypher queries and schemas into induced SQL queries and schemas before feeding them into \verieql.
%     % \item A \emph{transpiler optimizer.} 
% \end{itemize}




==> stale/stale-methodology.tex <==
\section{Generalization to Arbitrary Relational Schemas} \label{stale-sec:methodology}


In the previous section, we showed how a graph database can be migrated to a relational database: In particular, the concept of SST allows porting the ``data'' portion, whereas our syntax-directed translation rules allow migrating the ``query'' portion. However, the methodology proposed so far has one major limitation, namely that the \emph{induced relational schema} may be different from the  desired target schema. In this section, we show how to  handle cases where the target relational schema differs from the induced relational schema. 

\subsection{Specifying Schema Transformers}

Recall that the definition of equivalence between graph and relational databases inherently relies on the notion of a \emph{schema transformer} that describes the relationship between the graph and relational schemas. Thus, to generalize our approach to arbitrary relational schemas, we need a domain-specific language (DSL) for defining suitable transformers. 


% \input{figures/fig-trans-syntax}

Our observation is that this schema transformer DSL actually corresponds to a small fragment of the Cypher language.
In particular, recall that a Cypher query takes as input a graph database instance and produces a table. Given that a relational database is nothing but a set of tables, we can express the desired transformer using a \emph{set} of Cypher queries, one for each table in the target relational schema.
Since the entire Cypher query language is an overkill for specifying most schema transformers of interest, we only consider the subset of Cypher that includes simple pattern matching, filtering, and union operations.
The syntax of our schema transformer DSL is shown in Figure~\ref{fig:trans-syntax}.
We believe that this design choice optimizes both user-friendliness {and} expressivity:
instead of having to work with a new DSL, the user can simply use a familiar query language, namely Cypher, to specify the transformer $\transformer$. Furthermore, this subset of Cypher is sufficiently powerful for  expressing schema transformers of practical interest.


%Our observation is that Cypher itself is precisely such a DSL! In particular, recall that a Cypher query takes as input a graph database instance and produces a table. Given that a relational database is nothing but  of a set of tables, we can express the desired transformer using a \emph{set} of Cypher queries, one for each table in the target relational schema.  While the entire Cypher query language could be an overkill for specifying most schema transformers of interest, we believe that this design choice optimizes both  user-friendliness \emph{and} expressivity: instead of having to work with a new DSL, the user can simply use the Cypher language for specifying $\Phi$. Furthermore, while Cypher allows for expressing complex schema transformations, easier  transformations can also be expressed using a set of simple queries in a subset of Cypher.



%{In our approach, the user can specify the schema transformer $\Phi$ (as illustrated in Figure~\ref{fig:sst-rst-diagram}) via a \emph{set of Cypher queries}. The insight is that each Cypher query may be viewed as a property graph-to-table transformation. A relational database instance is exactly a collection of tables, thus a set of Cypher queries, when applied to the same input graph database instance, yields a relational database instance (and a corresponding relational database schema). In our case, we require the set of Cypher queries specifying $\Phi$ must yield a relational database instance $D$ such that $D \conform \Psi_R$ as output.


% SQL: Moive, BadMoive
% Cypher: MOIVE
% RETURN(Match(m1:Moive, top), [m1.id, m1.title], [m1.id, m1.title]) = RETURN(Match(m2:MOIVE, top), [m2.id, m2.title], [m2.id, m2.title])
% RETURN(Match(m2:BadMoive, top), [m2.id, m2.title], [m2.id, m2.title]) = RETURN(Match(m2:MOIVE, m2.bad_movie = top), [m2.id, m2.title], [m2.id, m2.title])

\begin{example}
Let $\gschema$ be a graph schema containing a \texttt{MOVIE} node with property keys \texttt{id}, \texttt{title}, and \texttt{good}, which store the identifier and title of a movie, as well as whether the movie is good or not.
Let $\rschema$ be the target relational schema consisting of two tables: \texttt{Movie(id, title)} and \texttt{GoodMovie(id, title)}, which store the information of all movies and good movies, respectively.
The schema transformer from $\gschema$ to $\rschema$ can be specified as follows:
\[
\begin{array}{rcl}
\texttt{Movie} & \gets & \sfReturn(\sfMatch([m, \texttt{MOVIE}], \top), [\texttt{m.id}, \texttt{m.title}], [\texttt{id}, \texttt{title}]) \\
\texttt{GoodMovie} & \gets & \sfReturn(\sfMatch([m, \texttt{MOVIE}], \texttt{m.good} = \emph{true}), [\texttt{m.id}, \texttt{m.title}], [\texttt{id}, \texttt{title}]) \\
\end{array}
\]
It corresponds to the following set of Cypher queries:
\[
\begin{array}{rcl}
\texttt{Movie} & \gets & \boldMatch \ (m:\texttt{MOVIE}) \ \boldReturn \ m.\texttt{id}, m.\texttt{title} \\
\texttt{GoodMovie} & \gets & \boldMatch \ (m:\texttt{MOVIE}) \ \boldWhere \ m.\texttt{good} = \text{true} \ \boldReturn \ m.\texttt{id}, m.\texttt{title} \\
\end{array}
\]
\end{example}

%\yang{The first Cypher query returns a list of tuples consisting of the property keys \texttt{id} and \texttt{title} from the $\mathsf{MOVIE}$ nodes which are equal to the relational table $\mathsf{Movie}$. To represent $\mathsf{BadMovie}$ is a sub-table of $\mathsf{Movie}$, the second Cypher query first filter out $\mathsf{MOVIE}$ nodes whose value of the property key \texttt{m.bad\_movie} is false, and let the result of this Cypher query equal to the relational table $\mathsf{BadMovie}$.}



%Until now, we have proposed a sound translation of both the "data`` part of Cypher into SQL (via an SST) and the "query`` part of Cypher into SQL (via the syntax-directed translation rules presented in the previous section). In this section, we discuss (1) how the user specifies the graph-to-relational schema transformer and (2) how we infer a residual schema transformer between the induced relational schema of the input graph schema.

\subsection{Verification Methodology}

% \input{figures/fig-sst-rst-diagram}

% \input{figures/algo-verify}

Now that we have a means of expressing the desired schema transformer $\transformer$, we turn our attention to verifying equivalence between a pair of Cypher and SQL queries that operate over database instances related through $\transformer$. In particular, suppose that we are given a Cypher query $Q_G$ over graph database schema $\gschema$ and a SQL query $Q_R$ over relational schema $\rschema$, and the relationship between the schemas is given by $\transformer$. Figure~\ref{fig:sst-rst-diagram} presents a diagram that illustrates our approach to verifying equivalence between $Q_G$ and $Q_R$.
More specifically, our verification methodology is shown in Algorithm~\ref{algo:verify}.
First, we compute the induced relational schema $\schema_{R'}$ of graph schema $\gschema$ and obtain the corresponding schema mapping $\smapping$ and SST $\sdt$ based on Definitions~\ref{def:irs} and \ref{def:sst} (Lines 2 -- 3).
Then we rewrite the given Cypher query $Q_G$ to a SQL query $Q_{R'}$ over the induced relational schema $\schema_{R'}$ of $\gschema$ (Lines 4 -- 5). Due to the correct-by-construction nature of our translation rules, we know that $Q_G$ and $Q_{R'}$ are equivalent modulo the SST $\sdt$. Now, to check whether $Q_G$ and $Q_R$ are equivalent, we can simply check equivalence between $Q_R$ and $Q_{R'}$ using existing equivalence checking techniques, such as ~\cite{verieql-oopsla24,mediator-popl18,cosette},  targeting SQL queries. However, since $Q_R$ and $Q_{R'}$ operate over potentially different relational schemas, we need to infer a schema transformer $\transformer'$ between $\rschema$ and $\schema_{R'}$ such that $\transformer = \transformer' \circ \sdt$. Fortunately, since $\sdt$ is invertible, we have $\transformer' = \transformer \circ \sdt^{-1}$; we refer to $\transformer'$ as the \emph{residual schema transformer} (Line 6).  Thus, we can verify equivalence between queries $Q_G$ and $Q_R$ by checking $Q_{R'} \simeq_{\transformer'} Q_R $ using existing techniques (Line 7). 

\begin{theorem}[Soundness]\label{thm:full-soundness}
Let $Q_G$ be a Cypher query over graph schema $\gschema$, $Q_R$ be a SQL query over relational schema $\rschema$, and $\transformer$ be a schema transformer.
Suppose that \textsf{CheckSQLEquivalence} is a sound procedure, if $\textsc{Verify}(\gschema, Q_G, \rschema, Q_R, \transformer)$ returns $\top$, it holds that $Q_G \simeq_{\transformer} Q_R$.
\end{theorem}
% \begin{proof}
% See the appendix under supplementary materials.
% \end{proof}


\begin{theorem}[Completeness]\label{thm:full-completeness}
Let $Q_G$ be a Cypher query over graph schema $\gschema$, $Q_R$ be a SQL query over relational schema $\rschema$, and $\transformer$ be a schema transformer.
Suppose that \textsf{CheckSQLEquivalence} is a complete procedure, if $Q_G \simeq_{\transformer} Q_R$, then $\textsc{Verify}(\gschema, Q_G, \rschema, Q_R, \transformer)$ returns $\top$.
\end{theorem}
% \begin{proof}
% See the appendix under supplementary materials.
% \end{proof}



\vspace{-5pt}

\bfpara{Remark.} In this discussion, we focus on checking equivalence between graph and relational queries; however, please note that the same methodology can also be used for 
transpiling a Cypher query to a SQL query, even when the desired relational schema $\rschema$ is different from the induced relational schema $\schema_{R'}$. In particular, once we have a SQL query $Q_{R'}$ over the relational schema, we can use the same residual schema transformer $\transformer'$ to synthesize a query $Q_R$ over $\rschema$ using existing SQL query synthesis techniques, such as~\citet{migrator-pldi19}.

%A diagram illustrating the relationships between schemas, queries, and schema transformers in our equivalence checking problem is shown in Figure~\ref{fig:sst-rst-diagram}. The graph schema $\schema_G$, relational schema $\schema_R$, queries $Q_G$ and $Q_R$, along with the graph-to-relational schema transformer $\Phi$ are provided as input to our equivalence checker by the user. The schema $\Psi_{R'}$ is the relational schema induced by applying the SST $\Phi_{\mathsf{sst}}$ on $\Phi_G$. The query $Q_{R'}$ is obtained through our syntax-directed query translation rules; one may think of it as composing the inverse SST $\Phi_{\mathsf{sst}}^{-1}$ with the Cypher query $Q_G$.

%Finally, the query equivalence problem asks us to check whether the two output tables $T_G$ (obtained from running the Cypher query $Q_G$ on a property graph $G \conform \schema_G$) and $T_R$ (obtained from running the SQL query $Q_R$ on a relational database instance $D \conform \schema_R$) are equivalent using the equivalence relation $\equiv$ (Definition~\ref{def:tableEquivalence}). By using the SST $\Phi_\mathsf{sst}$ to construct an induced relational schema $\schema_{R'}$, our methodology reduces the overall problem to checking whether $T_{R'} \equiv T_{R}$ where $T_{R'}$ is the result of running the SQL query $Q_{R'}$ on an induced relational database instance $\reldb' \conform \schema_{R'}$, because by construction, $T_{R'} \equiv T_G$.

%We next present two remaining components of our approach, which are illustrated in Figure~\ref{fig:sst-rst-diagram}: (1) how the user specifies the schema transformer $\Phi$; (2) the construction of a residual schema transformer (RST) $\Phi'$ between the induced relational schema $\Psi_{R'}$ and the input relational schema $\Psi_R$. 
%Recall the definition for query equivalence (Definition~\ref{def:queryEquivalence}) requires a schema transformer $\Phi$ be provided as an input parameter. Therefore, in our definitions for the verification problem and the synthesis problem for arbitrary schemas (Definitions~\ref{def:verificationProblem} and~\ref{def:synthesisProblem}), we require the user to provide a schema transformer $\Phi$ as part of the input along with the graph schema $\schema_G$ and the relational schema $\schema_R$. Both the schemas and the user-specified schema transformer are shown in the left part of Figure~\ref{fig:sst-rst-diagram}. 

%Our methodology uses a standard schema transformer $\Phi_{\mathsf{sst}}$ to translate $\schema_G$ into an induced relational schema $\schema_{R'}$ (Section~\ref{ssec:sst}
%) and the query translation procedure (Section~\ref{ssec:queryTranslation})} to translate a Cypher query $Q_G$ with 
%\todo{TODO}


%\subsection{Residual Schema Transformer}

%\todo{Given a graph schema $\schema_G$, a relational schema $\schema_R$, and a schema transformer $\Phi$ between $\schema_G$ and $\schema_R$, the \emph{residual schema transformer} is a schema transformer $\Phi'$ between the relational schema $\schema_{R'}$ induced by applying the SST $\Phi_{\mathsf{sst}}$ to the graph schema $\schema_G$. Such an RST can be inferred by composing the inverse of the SST and the user-provided schema transformer $\Phi$. As depicted by Figure~\ref{fig:sst-rst-diagram} the RST, denoted by $\Phi'$, is a schema transformer between relational schemas $\Psi_{R'}$ and $\Psi_{R}$. Since the relational schema $\Psi_{R'}$ is the induced relational schema of $\Psi_{G}$, one can apply the inverse SST $\Phi_{\mathsf{sst}}^{-1}$ to a database instance conforming to $\Psi_{R'}$ to get a database instance conforming to $\Psi_{G}$. In other words, $\Psi_G$ is the induced schema of $\Psi_{R'}$ under $\Phi_{\mathsf{sst}}^{-1}$.  One can further compose $\Phi_{\mathsf{sst}}^{-1}$ with $\Phi$ to map a database instance $\reldb' \conform \Psi_{R'}$ to a database instance $\reldb \conform \Psi_{R}$. Thus one can infer the RST from $\Phi$ by noting that $\Phi' = \Phi_{\mathsf{sst}}^{-1} \circ \Phi$.}










==> stale/stale-tab-trans-judgments.tex <==
\begin{figure}
\scriptsize
\centering
\begin{tabular}{c|l}
\toprule
\textbf{Judgement} & \textbf{Description} \\ 
\midrule
$\smapping, \integrity \vdash Q \transquery Q'$ & A Cypher query $Q$ translates to SQL query $Q'$ given schema mapping $\smapping$ and integrity constraint $\integrity$ \\
$\smapping, \integrity \vdash C \transclause \mathcal{X}, Q'$ & A Cypher clause $C$ translates to variables $\mathcal{X}$ and SQL query $Q'$ given mapping $\smapping$ and integrity constraint $\integrity$ \\
$\smapping, \integrity \vdash PP \transpattern \mathcal{X}, Q'$ & A Cypher pattern $PP$ translates to variables $\mathcal{X}$ and SQL query $Q'$ given mapping $\smapping$ and integrity constraint $\integrity$ \\
$\smapping, \integrity \vdash E \transexpr E'$ & A Cypher expression $E$ translates to SQL expression $E'$ given schema mapping $\smapping$ and integrity constraint $\integrity$ \\
$\smapping, \integrity \vdash \pred \transpred \pred' $ & A Cypher predicate $\pred$ translates to SQL predicate $\pred'$ given schema mapping $\smapping$ and integrity constraint $\integrity$ \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\caption{Different judgments involved in query transpilation from Cypher to SQL.}
\label{tab:trans-judgments}
\vspace{-10pt}
\end{figure}


==> stale/stale-translation.tex <==
\section{Synthesis using Standard Schema Transformers} \label{stale-sec:translation}


The problem statements given in the previous section are parameterized over a user-provided schema transformer. In this section, we first consider a fixed schema transformer that we refer to as SST (short for \emph{standard schema transformer}). Intuitively, an SST is the ``closest'' relational representation of the graph database schema that represents each node and edge type as a relational table. Using this notion of an SST, we can synthesize a relational query that is, by construction, equivalent to the input graph query $Q$ modulo the SST. Once we have a relational representation of $Q$ over some schema, we can use existing automated reasoning tools for SQL to solve the verification and synthesis problems over arbitrary schemas. 

In this section, we first define the notion of \emph{standard schema transformer} for a given graph database schema $\gschema$ and then present syntax-directed translation rules to transpile a given Cypher query over $\gschema$ to a SQL query using this SST. 



\subsection{Standard Schema Transformer} \label{ssec:sst}

For any graph database schema, we can  construct a corresponding relational schema by viewing each node and edge type as a table. We refer to this as the \emph{induced relational schema}:


\begin{definition}[\textbf{Induced relational schema}] \label{def:irs}
Given a database schema $\gschema = (T_N, T_E)$, we define its \emph{induced relational schema} $\rschema = (\tables, \integrity)$ and a corresponding  \emph{schema  mapping} $\smapping$ as follows:
\begin{itemize}[leftmargin=*]
\item For each $\nodeType = (l, K_1, \ldots, K_n) \in T_N$ with default property key $K_1$, there exists a relation $R_l \in \tables$ with attributes $K_1, \ldots, K_n$ and integrity constraint $\PK(R_l) = R_l.K_1$
such that $\smapping(l) = R_l$.
\item For each $\edgeType = (l, \stype, \ttype, K_1, \ldots, K_m) \in T_E$ with default property key $K_1$, there exists a relation $R_l \in \tables$ with attributes $K_1, ..., K_m, \fk_s, \fk_t$ and integrity constraint $\PK(R_l) = R_l.K_1 \land \FK(R_l.\fk_s) = \PK(\smapping(\stype)) \land \FK(R_l.\fk_t) = \PK(\smapping(\ttype))$. Additionally, we have $\smapping(l)= R_l$.
\end{itemize}
\end{definition}

\begin{example}\label{ex:irs}

Consider the graph schema $\gschema = (T_N, T_E)$ shown in Figure~\ref{fig:example-irs-graph}, where $T_N = \set{(\text{EMP}, \text{id}, \text{name}), (\text{DEPT}, \text{dnum}, \text{dname})}$ and $T_E = \set{(\text{WORK\_AT}, \text{EMP}, \text{DEPT}, \text{wid})}$. Its induced relational schema $\rschema = (\tables, \integrity)$ is visualized in Figure~\ref{fig:example-irs-relational}. Specifically, the induced relations are
\[
\tables = \set{\textbf{emp} \mapsto [\textrm{id}, \textrm{name}], \ \textbf{dept} \mapsto [\textrm{dnum}, \textrm{dname}], \ \textbf{work\_at} \mapsto [\textrm{wid}, \textrm{eid}, \textrm{did}]}
\]
The integrity constraint $\integrity$ is
\[
\begin{array}{rl}
 & \PK(\textbf{emp}) = \textbf{emp}.\textrm{id} \land \PK(\textbf{dept}) = \textbf{dept}.\textrm{dnum} \land \PK(\textbf{work\_at}) = \textbf{work\_at}.\textrm{wid} \\
\land & \FK(\textbf{work\_at}.\textrm{eid}) = \textbf{emp}.\textrm{id} \land \FK(\textbf{work\_at}.\textrm{did}) = \textbf{dept}.\textrm{dnum} \\
\end{array}
\]
And the schema mapping $\smapping$ is
\[
\smapping = \set{\textrm{EMP} \mapsto \textbf{emp}, \ \textrm{DEPT} \mapsto \textbf{dept}, \ \textrm{WORK\_AT} \mapsto \textbf{work\_at}} \\
\]

\input{figures/fig-example-irs}
\end{example}



Note that the schema mapping $\smapping$ given above can be used to define a schema transformer. We refer to this transformer associated with the induced schema as the \emph{standard schema transformer (SST)}.  In particular, if $\smapping$ maps a type to a relation $R$, then the SST converts all graph elements of this type to tuples in the corresponding relation:

\begin{definition}[\textbf{Standard schema transformer}]
\label{def:sst}
Let $G = (N, E, P, T)$ be a graph database instance over schema $\gschema$ with induced relational schema $\rschema$ and its corresponding mapping $\smapping$. Then, the SST $\sdt$ converts $G$ to a relational database as follows:
\begin{itemize}[leftmargin=*]
\item For each $n \in N$ with $T(n) = (l, K_1, \ldots, K_r)$, $\sdt$ creates a tuple $(K_1: P(n, K_1), \ldots, K_r: P(n, K_r)) \in \smapping(l)$.
\item For each $e = (n_s, n_t) \in E$ with $T(e) = (l, t_s, t_t, K_1, \ldots, K_m)$,  $T(n_s) = (l_s, K^s_1, \ldots K^s_m)$,  $T(n_t) = (l_t, K^t_1, \ldots K^t_j)$, $\sdt$ generates a tuple $(K_1: P(e, K_1), \ldots, K_m: P(e, K_m), K^s_1: P(n_s, K^s_1), K^t_1: P(n_t, K^t_1)) \in \smapping(l)$.
\end{itemize}
\end{definition}

Intuitively, $\sdt$ transforms each node with label $l$ to a tuple in the table $\smapping(l)$. 
For each edge with label $l$, $\sdt$ transforms it to a tuple in $\smapping(l)$ that includes values of all property keys associated with the edge, followed by the identifiers of the source and target nodes, respectively.

\begin{example} \label{ex:sst}
Consider the graph schema $\gschema$ in Example~\ref{ex:irs}. Let $G$ be a graph database instance (as visualized in Figure~\ref{fig:example-sst-graph}) that conforms to $\gschema$. We represent $G$  as a tuple $(N, E, P, T)$ where $N = \set{n_1, n_2, n_3, n_4}$, $E = \set{e_1 = (n_1, n_3), e_2 = (n_2, n_4)}$ and
\[
\begin{array}{rl}
P = \{ & (n_1, \textrm{id}) \mapsto 1, \ (n_1, \textrm{name}) \mapsto A, \ (n_2, \textrm{id}) \mapsto 2, \ (n_1, \textrm{name}) \mapsto B, \\
& (n_3, \textrm{dnum}) \mapsto 1, \ (n_3, \textrm{dname}) \mapsto CS, \ (n_4, \textrm{dnum}) \mapsto 2, \ (n_4, \textrm{dname}) \mapsto EE, \\
& (e_1, \textrm{wid}) \mapsto 10, \ (e_1, \textrm{eid}) \mapsto 1, \ (e_1, \textrm{did}) \mapsto 1, \ (e_2, \textrm{wid}) \mapsto 11, \ (e_2, \textrm{eid}) \mapsto 2, \ (e_2, \textrm{did}) \mapsto 1 \} \\
\end{array}
\]
\[
\begin{array}{rl}
T(n_1) = T(n_2) = & \hspace{-5pt} (\textrm{EMP}, \textrm{id}, \textrm{name}) \\
T(n_3) = T(n_4) = & \hspace{-5pt} (\textrm{DEPT}, \textrm{dnum}, \textrm{dname}) \\
T(e_1) = T(e_2) = & \hspace{-5pt} (\textrm{WORK\_AT}, \textrm{EMP}, \textrm{DEPT}, \textrm{wid}) \\
\end{array}
\]
Consider again the induced relational schema $\rschema$ and schema mapping $\smapping$ in Example~\ref{ex:irs}. The SST $\sdt$ converts $G$ to the relational database shown in Figure~\ref{fig:example-sst-relation}.
\input{figures/fig-example-sst}
\end{example}


\begin{theorem}[SST Invertibility]
\label{thm:sst-invertibility}
\footnote{Proofs of all the theorems can be found in the appendix under supplementary materials.
}
Let $\gschema$ be a graph schema and $\rschema$ be the induced relational schema. The standard schema transformer $\sdt$ from $\gschema$ to $\rschema$ is invertible.
\end{theorem}


\vspace{-5pt}
\bfpara{Remark.}
Let $\sdt$ be an SST. Given that $\sdt$ is invertible, we can use $\sdt^{-1}$ to generate a graph database instance from its relational representation.   



\subsection{Query Transpilation}
\label{ssec:queryTranslation}
Next, we describe how to transpile a Cypher query and obtain a correct-by-construction SQL query based on the schema mapping.




\bfpara{Intuition.}
To transpile a Cypher query to SQL, our key observation is that pattern matching in Cypher queries corresponds to a sequence of join operations in SQL queries. In particular, given schema mapping $\smapping$, 
a path pattern of form $n_1 \overset{e_1}{\rightarrow} n_2 \overset{e_2}{\rightarrow} ... \overset{e_{m-1}}{\rightarrow} n_m$ (where $n_i$ is a node pattern and $e_i$ is an edge pattern) in Cypher corresponds to the join of $\smapping(n_1), \smapping(e_2) \ldots,\smapping(e_{m-1}), \smapping(n_m)$ in SQL.
Based on this intuition, we develop a set of syntax-directed translation rules for transpiling Cypher queries to SQL queries. 

\bfpara{Judgments used in the transpilation procedure.} Before we explain the translation procedure in detail, we first give a high-level overview of the judgements used in this procedure which are summarized in Table~\ref{tab:trans-judgments}.  
\input{figures/tab-trans-judgments}
The top-level judgment is of the form $\smapping, \integrity \vdash Q \transquery Q'$ and is used for translating Cypher query $Q$  over schema $\schema$ to a relational query $Q'$ over the induced relational schema of $\schema$ given schema mapping $\smapping$ and integrity constraint $\integrity$. Similarly, judgments of the form $\smapping, \integrity \vdash E \transexpr E'$ and $\smapping, \integrity \vdash \phi \transpred \phi'$ are used for translating expressions and predicates respectively. On the other hand, the judgments for translating Cypher clauses and path patterns have a slightly different shape: Each clause and path pattern is translated to a corresponding SQL query $Q'$, along with a set of variable names (and their corresponding type) $\Xset$ that are introduced by the corresponding Cypher clause/pattern. Intuitively, our translation rules need to keep track of variable names/types in each pattern, as they affect how to perform joins correctly when translating nested matching clauses.




\input{figures/fig-trans-query}

\bfpara{Translating queries.}
The top-level rules for translating queries are shown in Figure~\ref{fig:trans-query} using judgments of the form $\smapping, \integrity \vdash Q \transquery Q'$, denoting that  Cypher query $Q$ translates to SQL query $Q'$. Among these rules, the most involved ones are for $\sfReturn$.
Specifically, if there is no aggregation function in $\overline{E}$, the \textrm{Q-Ret} rule translates the Cypher query $\sfReturn(C, \overline{E}, \overline{k})$ to a simple SQL query $\proj_{\rename_{\overline{k}}(\overline{E'})}(Q)$ that projects out the attribute expressions $\overline{E'}$ and renames all attributes to $\overline{k}$, where $Q$ is translated from Cypher clause $C$ and $\overline{E'}$ is translated from expression $E$.

If there is an aggregation function in $\overline{E}$, the \textrm{Q-Agg} rule translates $\sfReturn(C, \overline{E}, \overline{k})$ to a \texttt{GroupBy} query in SQL. In particular, the SQL query first groups the result of $Q$ based on all non-aggregation expression $\overline{A}$, where $Q$ is the translated query of clause $C$. Then it projects out all translated expressions $\overline{E'}$ and renames the attributes to $\overline{k}$.
Other Cypher queries including $\sfOrderBy$, $\sfUnion$, and $\sfUnionAll$ are translated to their corresponding SQL operations $\ttOrderBy$, $\cup$, and $\uplus$, respectively.

\begin{example} \label{ex:query}
Given the schema mapping $\smapping$ and integrity constraint $\integrity$ in Example~\ref{ex:irs}, let us consider the the Cypher query in Example~\ref{example:cypher1}:
\[
\sfReturn(\sfMatch([(\texttt{n}, \texttt{EMP}), (\texttt{e}, \texttt{WORK\_AT}, \rightarrow), (\texttt{m}, \texttt{DEPT})], \top), [\texttt{m.dname}, \sfCount(\texttt{n.id})], [\texttt{name}, \texttt{num}])
\]
Since there is a $\sfCount$ aggregation in the return query, we can apply the \textrm{Q-Agg} rule to translate it to a \ttGroupBy query in SQL.
Specifically, we first apply the \textrm{C-Match1} rule to translate the match clause $\sfMatch([(\texttt{n}, \texttt{EMP}), (\texttt{e}, \texttt{WORK\_AT}, \rightarrow), (\texttt{m}, \texttt{DEPT})], \top)$ into a SQL query $Q$ (explained in Example~\ref{ex:clause}).
Then we translate the returned Cypher expressions \texttt{m.dname} and $\sfCount(\texttt{n.id})$ to their corresponding SQL expressions \texttt{m.dname} and $\ttCount(\texttt{n.id})$. Among these expressions, we find the one that does not contain aggregations, namely \texttt{m.dname}, and use it as the grouping key for \ttGroupBy. Since there is no filtering based on the aggregated results, the \ttHaving clause for \ttGroupBy is not generated.
Therefore, the translated SQL query is 
$\ttGroupBy(Q, [\mathtt{m.dname}], \rename_{[\mathtt{name}, \mathtt{num}]}([\mathtt{m.dname}, \mathtt{Count(n.id)}]), \top)$.
\end{example}

\input{figures/fig-trans-clause}

\bfpara{Translating clauses.}
The rules for translating clauses are shown in Figure~\ref{fig:trans-clause}, where judgments of the form $\smapping, \integrity \vdash C \transclause \Xset, Q'$ denote that a Cypher clause is translated to a SQL query $Q'$ and all node and edge variables used in the clause are $\Xset$. Our translation rules for \boldMatch and \boldOptMatch in Cypher follow our earlier observation that  graph pattern matching in Cypher can be emulated through a sequence of join operations in SQL. 
Specifically, the \textrm{C-Match1} rule translates a simple match $\sfMatch(PP, \pred)$ to $\filter_{\pred'}(Q)$ where $Q$ is translated from the path pattern $PP$ and $\pred'$ is translated from the predicate $\pred$.
The \textrm{C-Match2} rule is more involved due to the potentially nested matching clauses. In particular, given a clause $\sfMatch(C, PP, \pred)$, \textrm{C-Match2} first translates the clause $C$ and path pattern $PP$ to obtain subqueries $Q_1$ and $Q_2$, respectively. It also collects all node or edge variables that are used in $C$ as $\Xset_1$ and used in $PP$ as $\Xset_2$. Then it finds all common variables in $\Xset_1, \Xset_2$ and, for each variable $X$ of type $l$, it generates  the join predicate $T_1.\integrity_{pk}(\smapping(l)) = T_2.\integrity_{pk}(\smapping(l))$ where $\integrity_{pk}(\smapping(l))$ denotes the primary key for relation type $\smapping(l)$.
This ensures that two different copies of a tuple obtained from the translation of $C$ and $PP$ are joined together correctly, i.e., they use the same primary key.
The \textrm{C-OptMatch} rule is very similar to \textrm{C-Match2}, but the difference is that the translated SQL query uses a left join instead of an inner join to add null values for missing tuples.
The \textrm{C-With} rule simply translates $\sfWith(C, \overline{Y}, \overline{Z})$ to a renaming SQL query $\proj_{\rename_{L[\overline{Z}/\overline{Y}]}(L)}(Q)$ that replaces all old names $\overline{Y}$ with new names $\overline{Z}$.

\begin{example} \label{ex:clause}
Given the schema mapping $\smapping$ and integrity constraint $\integrity$ in Example~\ref{ex:irs}, let us consider the Cypher clause $\sfMatch([(\texttt{n}, \texttt{EMP}), (\texttt{e}, \texttt{WORK\_AT}, \rightarrow), (\texttt{m}, \texttt{DEPT})], \top)$ in Example~\ref{example:cypher1}.
Based on the \textrm{C-Match1} rule, we need to use the \textrm{PT-Path} rule to collect all node and edge variables in the pattern, namely $\Xset = \set{(\texttt{n}: \texttt{EMP}), (\texttt{e}: \texttt{WORK\_AT}), (\texttt{m}: \texttt{DEPT})}$, and translate the pattern to a SQL query $\rename_{\mathtt{n}}(\mathtt{emp}) \ijoin_{\mathtt{n.id} = \mathtt{e.eid}} \rename_{\mathtt{e}}(\mathtt{work\_at}) \ijoin_{\mathtt{e.did} = \mathtt{m.dnum}} \rename_{\mathtt{m}}(\mathtt{dept})$. We also need to use the \textrm{P-True} rule to translate the Cypher predicate $\top$ to SQL predicate $\top$. Thus, the Cypher clause is translated to a SQL query $\filter_{\top}(\rename_{\mathtt{n}}(\mathtt{emp}) \ijoin_{\mathtt{n.id} = \mathtt{e.eid}} \rename_{\mathtt{e}}(\mathtt{work\_at}) \ijoin_{\mathtt{e.did} = \mathtt{m.dnum}} \rename_{\mathtt{m}}(\mathtt{dept}))$.
\end{example}

\input{figures/fig-trans-pattern}

\bfpara{Translating patterns.}
The rules for translating patterns are shown in Figure~\ref{fig:trans-pattern}. Similar to clauses, judgments for patterns are of the form $\smapping \vdash PP \transpattern \Xset, Q'$, denoting that a pattern $PP$ is translated to a SQL query $Q'$ and all node and edge variables used in the pattern are $\Xset$.
There are only two kinds of patterns. The first kind is a node pattern of the form $(X, l)$, the \textrm{PT-Node} rule simply collects the node variable $X$ of type $l$ and generates a SQL query $\rename_X(\smapping(l))$ that renames the relation $\smapping(l)$ to $X$.
The second kind is a path pattern of the form $(X_1, l_1), (X_2, l_2, d_2), PP$ where $PP$ is a sub-pattern. The \textrm{PT-Path} rule collects $X_1$, $X_2$, and the variable set $\Xset$ from $PP$ as the new variable set. It translates the path pattern to a SQL query $\rename_{X_1}(\smapping(l_1)) \ijoin_{\pred} \rename_{X_2}(\smapping(l_2)) \ijoin_{\pred'} Q'$ where $Q'$ is translated from the sub-pattern $PP$, which basically joins all tables corresponding to nodes and edges occurred in the path pattern. Again, this adheres to  our earlier observation that pattern matching in Cypher corresponds to a sequence of join operations in SQL.


\begin{example}
Given the schema mapping $\smapping$ and integrity constraint $\integrity$ in Example~\ref{ex:irs}, let us focus on the path pattern $[(\texttt{n}, \texttt{EMP}), (\texttt{e}, \texttt{WORK\_AT}, \rightarrow), (\texttt{m}, \texttt{DEPT})]$.
According to the \textrm{PT-Path} rule, we first need to apply the \textrm{PT-Node} rule to get the variables $\set{(\texttt{m} : \texttt{DEPT})}$ and query $\rename_{\texttt{m}}(\texttt{DEPT})$ from the node pattern $(\texttt{m}, \texttt{DEPT})$. Based on these results, we can use the \textrm{PT-Path} rule to collect all variables $\Xset = \set{(\texttt{n} : \texttt{EMP}), (\texttt{e} : \texttt{WORK\_AT}), (\texttt{m} : \texttt{DEPT})}$ and obtain the SQL query $\rename_{\mathtt{n}}(\mathtt{emp}) \ijoin_{\mathtt{n.id} = \mathtt{e.eid}} \rename_{\mathtt{e}}(\mathtt{work\_at}) \ijoin_{\mathtt{e.did} = \mathtt{m.dnum}} \rename_{\mathtt{m}}(\mathtt{dept})$.
\end{example}



\begin{theorem}[Soundness of translation]\label{lem:soundness}
Let $\gschema$ be a graph schema and $Q$ be a Cypher query over $\gschema$. Let $\rschema = (S, \integrity)$ be the induced relational schema of $\gschema$, $\smapping$ be the corresponding schema mapping, and $\sdt$ be the standard schema transformer from $\gschema$ to $\rschema$. If $\smapping, \integrity \vdash Q \transquery Q'$, then $Q'$ is equivalent to $Q$ modulo $\sdt$, i.e., $Q \simeq_{\sdt} Q'$.
\end{theorem}


\begin{theorem}[Completeness of translation] \label{thm:completeness}
Let $\gschema$ be a graph schema, $\rschema = (S, \integrity)$ be the induced relational schema of $\gschema$, and $\smapping$ be the corresponding schema mapping. Given any Cypher query $Q$ over $\gschema$ accepted by the grammar shown in Figure~\ref{fig:cypher-syntax}, there exists a SQL query $Q'$ over $\rschema$ such that $\smapping, \integrity \vdash Q \transquery Q'$.
\end{theorem}



==> stale/tab-statistics-schema-sql.tex <==
\begin{table}[!t]
\scriptsize
\centering
\caption{Statistics of relational schemas and SQL queries in benchmarks. \#Rel denotes the number of relations. \#Attr denotes the number of attributes}
\vspace{-10pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|cccc|cccc|cccc}
\toprule
\multirow{3}{*}{Dataset} & \multirow{3}{*}{\#} & \multicolumn{8}{c|}{Relational Schema}                  & \multicolumn{4}{c}{\multirow{2}{*}{SQL Size}} \\ \cline{3-10}
                         &                     & \multicolumn{4}{c|}{\#Rel} & \multicolumn{4}{c|}{\#Attr} & \multicolumn{4}{c}{} \\ \cline{3-14}
&                     & Min  & Max  & Avg  & Med  & Min   & Max  & Avg  & Med  & Min         & Max         & Avg         & Med        \\ 
\midrule
\stackoverflow & 12 & 1      & 5     & 2.3     & 2      & 2     & 11      & 5.8     & 5     & 15     & 74     & 32.5     & 28  \\
\tutorial & 26 & 1      & 4     & 2.3     & 2.5     & 2      & 12     & 6.3     & 5.5     & 5     & 76     & 25.8     & 22  \\
\academic & 7 & 3      & 5     & 4.7     & 5     & 10      & 12     & 11.0     & 11     & 27     & 59     & 46.9         & 54  \\
\hline
Total & 45 & 1      & 5     & 2.7     & 3     & 2      & 12     & 6.9     & 6     & 5     & 76     & 30.8         & 38  \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\label{tab:statistics-schema-sql}
\end{table}

